CompactTag: Minimizing Computation Overheads in Actively-Secure MPC for Deep Neural Networks

Secure Multiparty Computation (MPC) protocols enable secure evaluation of a circuit by several parties, even in the presence of an adversary who maliciously corrupts all but one of the parties. These MPC protocols are constructed using the well-known secret-sharing-based paradigm (SPDZ and SPDZ2k), where the protocols ensure security against a malicious adversary by computing Message Authentication Code (MAC) tags on the input shares and then evaluating the circuit with these input shares and tags. However, this tag computation adds a significant runtime overhead, particularly for machine learning (ML) applications with numerous linear computation layers such as convolutions and fully connected layers. To alleviate the tag computation overhead, we introduce CompactTag, a lightweight algorithm for generating MAC tags specifically tailored for linear layers in ML. Linear layer operations in ML, including convolutions, can be transformed into Toeplitz matrix multiplications. For the multiplication of two matrices with dimensions T1 x T2 and T2 x T3 respectively, SPDZ2k required O(T1 x T2 x T3) local multiplications for the tag computation. In contrast, CompactTag only requires O(T1 x T2 + T1 x T3 + T2 x T3) local multiplications, resulting in a substantial performance boost for various ML models. We empirically compared our protocol to the SPDZ2k protocol for various ML circuits, including ResNet Training-Inference, Transformer Training-Inference, and VGG16 Training-Inference. SPDZ2k dedicated around 30% of its online runtime for tag computation. CompactTag speeds up this tag computation bottleneck by up to 23x, resulting in up to 1.47x total online phase runtime speedups for various ML workloads.

==> archives/0.abstract.tex <==
\begin{abstract}
Many Multi-Party Computation (MPC) protocols, such as SPDZ~\cite{somewhatMAC}, Overdrive~\cite{overdrive}, MASCOT~\cite{mascot}, and SPD$\nZ_{2^k}$~\cite{spdz2k}, allow secure evaluation of complex circuits in the active adversarial setting (dishonest majority). These protocols generate information-theoretical MACs (IT MACs) for operands involved in the computation, providing a mechanism to verify the correctness of the final results. Consequently, during the online phase, each party computes the secret share of the final result and the secret share of the IT MACs corresponding to that result. This additional MAC computation contributes to a significant portion of the online phase runtime, especially for workloads with large matrices such as Machine Learning (ML). For ML workloads, most of the operands are large matrices, and each large matrix is associated with an IT MAC of the same dimension. These large IT MACs amplify the computational cost, making the process of IT MAC computation more resource-intensive.

To mitigate the added MAC computation during the online phase, in this paper, we introduce \name{}, a novel lightweight algorithm to generate IT MACs for large matrix operations. Our novel IT MAC generation algorithms can speed up ML inference and training by 1.31x and 1.4x, respectively, over SPD$\nZ{2^k}$, the state-of-the-art actively secure dishonest majority MPC.
\end{abstract}

==> archives/1.introduction.tex <==
\section{Introduction}
Multi-Party Computation (MPC) allows a set of $n$ parties $\{\party{i}\}_{i=1}^{n}$ to collectively evaluate a function $r = f(x, y, ...)$ while keeping inputs private. MPC keeps inputs private by creating secret shares of the input values over a ring or a finite field. Thus, instead of holding inputs $(x, y, ...)$ directly, $\party{i}$ will hold secret shares $(\as{x}{i}, \as{y}{i}, ...)$, where $(x, y, ...)$ can only be reconstructed using $(\as{x}{i}, \as{y}{i}, ...)$ from a subset of participating parties. In this way, no party can learn the original operand without some parties colluding. Then, MPC parties can then securely evaluate the function $r = f(x, y, ...)$. Most MPC protocols follow the online/offline phase setting. During the offline phase, slow but input-independent computations, such as Beaver Triple generation and secret share authentication, are performed. During the online phase, input-dependent computations are performed. When one deploys MPC computations as a service, the online phase is most pertinent to computation latency when inputs arrive.


\paragraph{MPC Security Model:} The security of MPC is usually measured by two dimensions: 1) the maximum number of corrupted parties and 2) the power of the adversaries. Given a set of $n$ parties $\{\party{i}\}_{i=1}^{n}$, if an MPC protocol can tolerate more than or equal to $n / 2$ parties, the MPC protocol is secure against dishonest majority, otherwise honest majority. As for the power of the adversary, the adversary is considered a passive adversary if the adversary follows the exact protocol but is curious about the input operands. On the other hand, an active adversary might not follow the protocol and will try to breach both the privacy and the correctness of MPC protocols. This paper will focus on \textit{actively secure dishonest majority MPC}.

\paragraph{Actively Secure MPC Overheads:} Actively secure MPC protocols need to verify the computational outputs to guard against adversaries. These protocols generate element-wise information-theoretical MAC tags (IT MACs)for all the participating elements. For example, a $[\sizem \cross \sizen]$ matrix operand will have a $[\sizem \cross \sizen]$ IT MAC. When computing the final results during the online phase, the operations that were applied to the secret shares are usually repeated on the IT MACs. This ensures that any new computed value will have an IT MAC to check the correctness, enabling the participating parties in the MPC to verify the final results. IT MACs, however, introduce significant computation demands during the online phase. Thus, a noticeable portion of online phase runtime in actively secure dishonest majority settings is IT MAC-related operations. Our system spends approximately $16\%$ to $28\%$ of the online phase on tag-related computations. It is, thus, known that the online phase of MPC protocols that are secured against active and dishonest majority adversaries have the highest overheads than  MPC protocols that guard against passive adversaries. 

% These IT MACs will need truncation (more on this in later sections). Truncation of IT MACs induces additional communication. The added IT MAC operation is even more acute for ML workloads as most operands to ML are large matrices. 

\subsection{Our Contribution}
(1)  In this paper, we design a novel online phase matrix multiplication and Convolution algorithm. These algorithms minimize IT MAC-related overheads of deep neural network (DNN) based ML workloads during the online phase of SPD$\nZ_{2^k}$, the state-of-the-art actively secure dishonest majority MPC protocol over rings. Unlike the state-of-art protocol for matrix multiplication and Convolution protocols, which mirrors computationally heavy matrix operations of secret shares values on IT MACs, \name{} algorithm allows MPC parties to obtain an IT MAC using cheaper operations. \name{} achieves this goal by first allowing MPC parties to obtain a tentative IT MAC for the final result using a passively secure protocol. This tentative IT MAC generation algorithm is passively secure and computationally lightweight. To verify the correctness of tentative IT MAC with little computation, we propose a novel IT MAC compression method, which reduces the IT MAC size by one dimension via random combinations along one axis. MPC parties will use our novel compression technique to compress their local operands. Those compressed operands will then later be used to compute a compressed version of the final matrix product. Due to the use of small compressed IT MACs, computation of the resulting small tag is also lightweight. The compressed small tag is then used to verify the correctness of the tentative IT MAC generated by the passively secure protocol. All algorithms we use for \name{}, tentative tag generation, and operand compression are all computationally lightweight. Thus, \name{} significantly reduces IT MAC generation overhead.

%YW: I THINK THE ABOVE PARAGRAPH NEEDS TO REWRITTEN MORE CLEANLY FOLLOWING THE ALGORITHMIC FLOW. LET US TALK, AND WE CAN DISCUSS HOW TO MAKE THIS CONTRIBUTION MORE CRIPS. 

(2) In addition to mitigating IT MAC-related computation costs, we also introduce a novel hybrid protocol that integrates matrix operations with truncation. This innovative approach ensures that the proposed tentative tag generation algorithm imposes zero overheads on both the online and offline phases. We first propose a stand-alone tentative tag generation algorithm that sacrifices another authenticated shared matrix. This stand-alone mechanism incurs increased communication costs during the online phase and demands extra preparation in the offline phase. However, our in-depth analysis discovered that the operations in our tentative tag generation algorithm are a subset of the operations in the state-of-art truncation protocols. Moreover, for ML workloads, operands are implemented using fixed-point representation. Thus, ML MPC multiplications, including matrix multiplications and Convolutions, are always followed by truncation operations. With these observations, we merge our tentative tag generation algorithm with the state-of-art truncation protocols. The resulting hybrid protocol eliminates the additional communication in the online phase and the additional authenticated share preparation in the offline phase.

(3) Finally, we implement \name{} and evaluate its efficiency for three major DNN models: 1) VGG16, 2) ResNet, and 3) Transformer. We show \name{} can reduce inference and training runtime and GPU power usage. \name{} reduces inference and training runtime up to $1.31$x and $1.40$x, respectively. \name{} reduced power consumption by $35\%$

\subsection{Notation}
In this section, we will describe the notation we use throughout this paper. We will use $v \in \TextRing$ to denote a value in modulo of $2^k$. We will use $\mM \in \TextRing^{\sizem \cross \sizen}$ to denote a $\sizem \cross \sizen$ matrix, and every element in such a matrix is in modulo of $2^k$. Given two matrix $\mM \in \TextRing^{\sizem \cross \sizen}$ and $\mY \in \TextRing^{\sizen \cross \sizeo}$, we use $\mM \mmul \mY$ to denote matrix multiplication. Given two matrices of the same size, $\mM \in \TextRing^{\sizem \cross \sizen}$ and $\mZ \in \TextRing^{\sizem \cross \sizen}$, we use $\mM \ewmul \mZ$ to denote element-wise multiplication between $\mM$ and $\mZ$, and we will use $\iprod{\mM}{\mZ}$ to denote inner products between matrix $\mX$ and $\mZ$. We use $\mac{v}$ and $\mac{\mM}$ to denote IT MAC for a value $v$ and matrix $\mM$, respectively. We will use $\as{v}{i}$, $\as{\mac{v}}{i}$, $\as{\mM}{i}$, and $\as{\mac{\mM}}{i}$ to denote the $\party{i}$'s local share of  value $v$, IT MAC of $v$, matrix $\mM$, and IT MAC of $\mM$, respectively. Any matrix symbol with an upper-right $'$ denotes the compressed version of that symbol. For instance, $\mM'$ signifies an operand compressed from $\mM$, while $\mac{\mM}'$ represents a compressed IT MAC associated with operand $\mM$. We will also abbreviate $x=y \mod 2^k$ as $x\modeq{k} y$.

\subsection{Overview of our protocol}

\paragraph{Online Phase:} In this section, we will use a matrix multiplication $\mZ = \mX \mmul \mY$,  where $\mX\in\TextRing^{\sizem \cross \sizen}$, $\mY\in\TextRing^{\sizen \cross \sizeo}$, and $\mZ \in \TextRing^{\sizem \cross \sizeo}$. Each matrix $\mX$ and $\mY$ will also have its own associated IT MAC. During the online phase, parties first compute their local share of $\mZ$. Then, parties will need to use the tentative tag generation algorithm to generate a new IT MAC tag for $\mZ$. After that, MPC parties will sample $\sizeo$ public random numbers. MPC parties will use those $\sizeo$ random numbers to invoke our tag compression algorithm to compress the tag of $\mY$ by performing random linear combination, such that the dimension of $\mY$'s compressed tag is $[\sizen \cross 1]$. Using this compressed small tag of $\mY$ and regular tag of $\mX$, MPC parties will compute a compressed small tag of $\mZ$ whose dimension is $[\sizem \cross 1]$. After that, MPC parties will use $\mZ$'s small tag to verify the correctness of $\mZ$'s tentative IT MAC. Note that our protocol works similarly to Convolution, except that the compression dimension of $\mY$ is the output channel of $\mY$. For other protocols, such as ReLU, MaxPooling, and truncation, we adhere to the same protocol detailed in the referenced work~\cite{spdz2k,spdk2kml}.


\paragraph{Tentative Tag Generation:} The tentative tag generation protocol is essential for our protocol. It allows our protocol to obtain a tentative regular IT MAC, which can be verified with a compressed small tag. Let's use a matrix $\mM$ as an example to illustrate our tentative tag generation algorithm. For the stand-alone version of such an algorithm, a random authenticated matrix $\mR$ whose size is the same as $\mM$ is prepared during the offline phase. With those inputs, MPC parties will open $\mR-\mM$ and use $\mR-\mM$ and the tag of $\mR$ to compute the tentative tag for $\mM$. This algorithm is only passively secure because adversaries can introduce errors to $\mR-\mM$. Thus, it is the actively secure protocols' responsibility, which use the tentative tag generation algorithm, to verify the correctness of $\mR-\mM$. This stand-alone algorithm introduces additional communication when opening $\mR-\mM$ and requires an authenticated random matrix $\mR$. Luckily, we have observed that the stand-alone tag generation algorithm is very similar to the truncation protocol. We propose a novel hybrid algorithm that performs truncation and tentative tag generation at the same time, such that they share the same pre-authenticated matrix $\mR$ and open the same $\mR-\mM$ in the online phase. In this way, our \name{} algorithms introduce no additional online phase communication and no additional offline phase preparation.


\paragraph{Offline Phase:} When using our most optimal hybrid \name{} algorithm, our offline phase requires no additional work. During the offline phase, when using \name{} algorithms, MPC parties behave exactly the same as if they are using algorithms in~\cite {spdz2k,spdk2kml}. 


\subsection{Related Work}
% \yongqin{Please add more related works if you see fit.}

The most relevant related works for our paper are SPD$\nZ_{2^k}$~\cite{spdz2k} and~\cite{spdk2kml}. SPD$\nZ_{2^k}$is the first to propose actively secure dishonest majority MPC over a ring. \cite{spdk2kml} described additional protocols, such as ReLU and truncation, used commonly in ML applications. Many of the protocols used in this paper are taken from both works. Yet, \name{} distinguishes itself by introducing innovative matrix multiplication and Convolution protocols. These new approaches leverage smaller compressed IT MACs to minimize online phase IT MAC-related overheads.  We propose a tag-related optimization to actively secure dishonest majority MPC.

SPDZ~\cite{somewhatMAC}, MASCOT~\cite{mascot}, and Overdrive~\cite{overdrive} are actively secure dishonest majority MPC over finite fields. \name{} can be easily applied to them by replacing ring-based sub-protocols in \name{} with finite filed-based sub-protocols. This work specifically focuses on ring-based protocols due to their faster performance in GPUs. The work of \cite{ACNS:BenNieOmr19} also proposed improvements by considering function-dependent preprocessing phases. 

There is a line of works \cite{EscuderoGPSW23,C:GoyPolSon22} in the weaker dishonest majority setting where a constant fraction $\epsilon$ (where $\tfrac{1}{2} < \epsilon < 1$) of the parties are corrupted by the adversary. In this setting, these works obtain efficient protocols based on packed secret sharing. Our protocol considers the stronger setting where the adversary can corrupt up to all but one party. 

There exists a plethora of works in online phase optimizations~\cite{reluMPC1, reluMPC2, reluMPC3, wangCharacIspass, crypten2020, aby2, mpc-pipe}, but those works mostly focus on the passive secure 2PC protocols whereas \name{} is designed for actively secure dishonest majority MPC. ~\cite{mpcformer} is a system-level optimization of Softmax specifically for MPC, which could be applicable to actively secure dishonest majority MPC.



%The VOLE protocol implementation is based on Moz$\nZ_{2^k}$arella~\cite{C:BBMS22}. 

\subsection{Paper organization}
This paper is organized as follows: In Section~\ref{sec:prelim}, we discuss this paper's necessary background information about SPD$\nZ_{2^k}$. In Section~\ref{sec:mainbody}, we will introduce our novel matrix multiplication and Convolution algorithms. Section~\ref{sec:security} shows security analysis \name{}. Section~\ref{sec:eval} evaluates \name{}. Section~\ref{sec:conclusion} concludes this paper.


==> archives/2.background.tex <==
\section{Preliminaries}
\label{sec:prelim}

% \subsection{Notations}
% \fixme{Provide general notations used in the paper for matrix multiplication}

\subsection{Background on SPD$\nZ_{2^k}$}
\paragraph{IT MAC Authentication:} To authenticate a given value $v\in \TextRing$ among a set of $n$ parties $\{\party{i}\}_{i=1}^{n}$. MPC parties will secretly share $v$ in the larger ring size of $2^{k+s}$, namely $\hat{v} \modeq{k+s} \sum_{i=1}^{n} \as{v}{i}$, and $v \modeq{k} \hat{v}$, where $\as{v}{i} \in \CipherRing$, and $s$ is the security parameter. Besides secretly shared value, there is a global key $\mkey{} \in \KeyRing$, and this global key is also additively shared among $n$ parties. The IT MAC of such value is $\mac{v} \modeq{k+s} \mkey{} \cdot \hat{v}$. This IT MAC of value $v$ is also secretly shared among $n$ parties. Thus, to secretly share a value $v$, parties need to hold the following operands:
\begin{align}
    (\as{v}{i}, \as{\mac{v}}{i}, \as{\mkey{}}{i})_{i=1}^{n} \in (\CipherRing \cross \MacRing \cross \KeyRing)^n
\end{align}
It is also easy to see that
\begin{align}
    \sum_{i=1}^{n} \as{\mac{v}}{i} \modeq{k+s} (\sum_{i=1}^{n} \as{v}{i}) \cdot (\sum_{i=1}^{n} \as{\mkey{}}{i})
\end{align}

Similarly, to secretly share a matrix $\mM \in \TextRing^{\sizem \cross \sizen}$, MPC parties will hold the following:
\begin{align}
    (\as{\mM}{i}, \as{\mac{\mM}}{i}, \as{\mkey{}}{i})_{i=1}^{n} \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen} \cross \KeyRing)^n \\
    \sum_{i=1}^{n} \as{\mac{\mM}}{i} = (\sum_{i=1}^{n} \as{\mM}{i}) \cdot (\sum_{i=1}^{n} \as{\mkey{}}{i}) \mod 2^{k+s}
\end{align} 


\paragraph{Single Check:} During MPC computations, opening a value that won't leak information about original operands is a common operation. In SPD$\nZ_{2^k}$, to open a value $v$, which is authenticated, MPC parties will perform the following procedure:
\begin{enumerate}
    \item Generated and authenticated random value $r\in \KeyRing$, such that each party will hold $\as{r}{} \in \CipherRing$ and $\as{\mac{r}}\in \MacRing$.
    \item Each $\party{i}$ computes $\as{w}{i} = \as{v+2^k\cdot r}{i}$, and its respective IT MAC $\as{\mac{w}}{i}$.
    \item Broadcast $\as{w}{i}$, such that each party will hold $w = \sum_{i=1}^{n} \as{w}{i} \mod 2^{k+s}$.
    \item Each $\party{i}$ computes $\as{u}{i} = \as{\mac{w}}{i} - w \cdot \asmac{i} \mod 2^{k+s}$.
    \item Broadcast $\as{u}{i}$ and check if $u = \sum_{i=1}^{n} \as{u}{i}$ equals zero.
    \item If $u$ equals zero, opened value $v$ is correct, otherwise abort.
\end{enumerate}


\paragraph{Batched Check:} The above checking scheme will fail with probability at most $2^{-s}$~\cite{spdz2k}. For ML workloads, it is not ideal to check a matrix of values individually due to added communication costs. A batched checking procedure is also proposed in SPD$\nZ_{2^k}$. Detailed procedure is described in Figure~\ref{fig:batchcheck}.



\begin{figure}[!t]
    \begin{framed}
    \centerline{\textbf{Procedure} $\procn{Batched Check}$}
    \smallskip

    \begin{flushleft}
    Procedure for opening a matrix $\mM \in \CipherRing^{\sizem \cross \sizen}$. The matrix $\mM$ is secretly shared and authenticated.\\
    
    \textbf{\textsc{Inputs:}} $\party{i}$ has a key $\asmac{i} \in \KeyRing$ and authenticated shares:\\
    \begin{itemize}
        \item  $(\as{\mM}{i}$, $\as{\mac{\mM}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$. \smallskip
        \item  $(\as{\mQ}{i}$, $\as{\mac{\mQ}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$. \smallskip
    \end{itemize}
    $(\as{\mQ}{i}$, $\as{\mac{\mQ}}{i})$ is obtained during the offline phase such that $\sum_{i=1}^{n} \as{\mQ}{i} \mod 2^k$ is a zero matrix.
    
    \textbf{\textsc{Open Phase:}} Open the matrix $\mM$:
    \begin{enumerate}
        \item Computes matrix $\as{\mW}{i} = \as{\mM}{i} +  \as{\mQ}{i}$, and its tag $\as{\mac{\mW}}{i} = \as{\mac{\mM}}{i} + \as{\mac{\mQ}}{i}$.
        \item Broadcast $\as{\mW}{i}$, such that every party obtains $\mW = \sum_{i=1}^{n} \as{\mW}{i} \mod 2^{k+s}$.        
    \end{enumerate}    


    \textbf{\textsc{Tag check phase: }} \\
    \begin{enumerate}
        \item All parties collectively sample a public random matrix $\chi \in \KeyRing^{\sizem \cross \sizen}$.
        \item $\party{i}$ computes $\as{cs}{i} \modeq{k+s} \iprod{\as{\mac{\mW}}{i}}{\chi} - \mkey{i} \cdot \iprod{\mW}{\chi}$.
        \item Each $\party{i}$ broadcast and compute $cs = \sum_{i}^{n} \as{cs}{i}$.
        \item All parties check if $cs \modeq{k+s}$. If the check fails, all parties abort the computation.
        % \item Each $\party{i}$ computes $\iprod{\mW}{\chi}$ and sums all the elements modulo $2^{k+s}$ in the resulting matrix to obtain $\mU \in \CipherRing^{\sizem \cross \sizen}$.
        % \item Each $\party{i}$ computes $\chi * \as{\mac{y}}{i}$ and sums all the elements modulo $2^{k+s}$ in the resulting tag matrix to obtain $\as{\mac{\mU}}{i} \in \CipherRing^{\sizem \cross \sizen}$.
        % \item Each $\party{i}$ computes and broadcast $\as{\mZ}{i} = \as{\mac{\mU}}{i} - \asmac{i} \cdot \mU$.
        % \item Each $\party{i}$ computes $\mZ = \sum_{i=1}^{n} \as{\mZ}{i} \mod 2^{k+s}$. If $\mZ$ is a zero matrix, opened matrix $\mM$ is correct. Otherwise, abort operations.
    \end{enumerate}

  \end{flushleft}
  %\vspace{-5mm}
  \end{framed}
\caption{Procedure of Batched Check.}
\label{fig:batchcheck}
\end{figure}

We can see that during the Tag Check Phase, MPC parties only broadcast one element value to check a matrix of values. The batched checking procedure above will only fail with probability at most $2^{-s+log(s+1)}$~\cite{spdz2k}.


\begin{figure}[!t]
    \begin{framed}
    \centerline{\textbf{Procedure} $\procn{MatMul}$}
    \smallskip

    \begin{flushleft}
    Procedure for performing $\mZ = \mX \mmul \mY$, where $\mZ\in  \TextRing^{\sizem \cross \sizeo}$, $\mX\in  \TextRing^{\sizem \cross \sizen}$, and $\mY\in  \TextRing^{\sizen \cross \sizeo}$. Matrices $\mX$ and $\mY$ are secretly shared and authenticated.\\
    
    \textbf{\textsc{Inputs:}} $\party{i}$ has a key $\asmac{i} \in \KeyRing$ and authenticated shares:\\
    \begin{itemize}
        \item  $(\as{\mX}{i}$, $\as{\mac{\mX}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$. \smallskip
        \item  $(\as{\mY}{i}$, $\as{\mac{\mY}}{i}) \in (\CipherRing^{\sizen \cross \sizeo} \cross \MacRing^{\sizen \cross \sizeo})$. \smallskip
        \item  $(\as{\mA}{i}$, $\as{\mac{\mA}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$. \smallskip
        \item  $(\as{\mB}{i}$, $\as{\mac{\mB}}{i}) \in (\CipherRing^{\sizen \cross \sizeo} \cross \MacRing^{\sizen \cross \sizeo})$. \smallskip
        \item  $(\as{\mC}{i}$, $\as{\mac{\mC}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$.
    \end{itemize}
    Authenticated shared matrix $\mA$, $\mB$, and $\mC$ are Beaver matrix triple such that: $\mC = \mA \mmul \mB$. This triple is obtained during the offline phase.

    \textbf{\textsc{Matrix Multiplication: }} \\
    \begin{enumerate}
        \item Each $\party{i}$ executes open phase of Batched Check to open $\as{\mX-\mA}{i}$ and $\as{\mY-\mB}{i}$ as $\mE$ and  $\mU$, respectively.
        \item $\party{i}$ computes locally $\as{\mZ}{i} = \as{\mC}{i} + \mE \mmul \as{\mB}{i} + \as{\mA}{i} \mmul \mU$.
        \item $\party{i}$ computes locally $\as{\mac{\mZ}}{i} = \as{\mac{\mC}}{i} + \mE \mmul \as{\mac{\mB}}{i} + \as{\mac{\mA}}{i} \mmul \mU$.
        \item $\party{i = 1}$ computes locally $\as{\mZ}{i} = \as{\mZ}{i} + \mE \mmul \mU$ and $\as{\mac{\mZ}}{i} = \as{\mac{\mZ}}{i} + \asmac{i} \cdot (\mE \mmul \mU)$
    \end{enumerate}

    \textbf{\textsc{Output: }} \\
    \begin{enumerate}
        \item Use the Tag Check Phase from the Batched Check to check the validity of opened values during matrix multiplication.
        \item If the previous step does not abort, output $(\as{\mZ}{}, \as{\mac{\mZ}}{})$ as authenticated shared of $\mZ = \mX \mmul \mY$.
    \end{enumerate}
  \end{flushleft}

  \end{framed}
\caption{Procedure of Matrix Multiplication in SPD$\nZ_{2k}$.}
\label{fig:mpcmatmul}
\end{figure}



\subsection{Secure ML Operations using MPC}
\label{sec:mlmpc}
In this section, we will discuss how common ML operations are implemented over a ring.

\paragraph{Fixed-Point:} Operands for ML workloads are real numbers. Fixed point encoding is the most accurate implementation of real numbers over rings. Fixed Point encoding scheme uses integers to represent fraction numbers. Fixed points will use trailing $p$ bits as precision bits. For example, if a value is $v$ as an integer, the value as a fixed point number is $\frac{v}{2^p}$.

% \fixme{Elaborate more and how are they performed?}

\paragraph{Matrix Multiplication:} Large matrix multiplications are widely used in applications like linear regression, Multi-level Perceptron, and Convolution Neural Networks. Let's use matrix multiplication $\mZ = \mX \mmul \mY$, where $\mZ\in  \TextRing^{\sizem \cross \sizen}$, $\mX\in  \TextRing^{\sizem \cross \sizen}$, and $\mY\in  \TextRing^{\sizen \cross \sizeo}$, as an example to illustrate how they are implemented in the MPC. Input operands $\mX$ and $\mY$ are secretly shared and authenticated among a set of MPC parties $\{\party{i}\}_{i=1}^{n}$. Thus, each party will hold a local share of matrix $\mX$ and its IT MAC. The state-of-art protocols for our threat model (actively secure and dishonest majority) use a secretly shared and authenticated Beaver Triple  $\mC\in \TextRing^{\sizem \cross \sizen}$,  $\mA\in \TextRing^{\sizem \cross \sizen}$, $\mB \in \TextRing^{\sizen \cross \sizeo}$, where $\mC = \mA \mmul \mB$, to facilitate matrix multiplication. Triples like those are obtained during the offline phase. During the online phase, MPC parties will then collectively compute secret shares of $\mZ$ and $\mZ$'s IT MAC. The detailed procedure for the online phase is described in Figure~\ref{fig:mpcmatmul}. 

Note that when opening (or batch checking) $\mE$ and $\mU$, we can omit $\mQ$ because $\mA$ and $\mB$ are in modulo $2^{k+s}$~\cite{spdz2k}. Thus, upper bits for $\mX$ and $\mY$ are already hidden by $\mA$ and $\mB$.

% To convert procedures in Figure~\ref{fig:mpcmatmul} to an MPC Convolution procedure, one simply needs to replace every matrix multiplication in Figure~\ref{fig:mpcmatmul} with a corresponding Convolution operation.


\paragraph{Convolution:} Convolution operations are also widely used in ML applications. Like matrix multiplication, Convolution is also a linear operation, and it can even be converted to matrix multiplications. Thus, the procedure for Convolution is similar to the matrix multiplication procedure described in Figure~\ref{fig:mpcmatmul}. To obtain an MPC Convolution procedure, one just needs to replace every matrix multiplication with Convolution in Figure~\ref{fig:mpcmatmul}.


\paragraph{Truncation Protocol:}
\label{sec:truncation}
For ML workloads, fixed-point encoding is commonly used to represent real numbers. When using fixed-point representation ($p$ bits are used for precision) to perform multiplication, the trailing $p$ bits of the products must be discarded. If we have a secret shared value, denoted as $\as{v}{}$, the most direct approach to drop the last $p$ bits is to have each MPC party locally divide $\as{v}{}$ by $l=2^p$.  However, this method would produce errors if the sum of secret shares $\as{v}{}$ wraps around the ring size of $Q$. Let's define $\theta_v$ as the count of wraps such that $v = \sum_i \as{v}{i} -\theta_vQ$. It becomes evident that this approach would fail when $\theta_v \neq 0$, as demonstrated by the inequality below.
\begin{align}
    \frac{v}{l} = \sum_i \frac{\as{v}{i}}{l} - \frac{\theta_v}{l}Q \neq \sum_i \frac{\as{v}{i}}{l} - \theta_vQ
\end{align}
Thus, when truncating IT MACs, we need to use a different approach. The truncation protocol we are using is the same as the one in~\cite{spdk2kml}. Figure~\ref{fig:macTruncation} describes the detailed procedure of matrix truncation. The probabilistic procedure in Figure~\ref{fig:macTruncation} will fail with probability at most $2^{-s}$.

\begin{figure}[!t]
    \begin{framed}
    \centerline{\textbf{Procedure} $\procn{Truncation}$}
    \smallskip

    \begin{flushleft}
    Procedure for truncating the last $p$ bits of an given authenticated shared matrix $(\as{\mM}{}, \as{\mac{\mM}}{})$.\\
    \textbf{\textsc{Inputs:}} $\party{i}$ has a key $\asmac{i} \in \KeyRing$ and authenticated secret shares: \\
    
    
    \begin{itemize}
        \item  $(\as{\mM}{i}, \as{\mac{\mM}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$. \smallskip
        \item  $(\as{\mR}{i}, \as{\mac{\mR}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$. \smallskip
        \item  $(\as{\hat{\mR}}{i}$, $\as{\mac{\hat{\mR}}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$.
    \end{itemize}
    where  $\hat{\mR} = \frac{\mR}{2^p}$, and authenticated shares of $\mR$ and $\hat{\mR}$ are obtained during the offline phase. \\
    \textbf{\textsc{Truncation: }} \\
    \begin{enumerate}
        \item Use the Open Phase of $\procn{Batched Check}$ to open $\as{\mR-\mM}{}$ as $\mD$.
        \item $\party{i}$ computes $\as{\mU}{i} = \as{\hat{\mR}}{i}  - \frac{\mD}{2^p}$.
        \item $\party{i}$ computes $\as{\mac{\mU}}{i} = \as{\mac{\hat{\mR}}}{i} - \asmac{i} \cdot \frac{\mD}{2^p}$.
    \end{enumerate}

    \textbf{\textsc{Output: }} \\
    \begin{enumerate}
        \item Use the Tag Check Phase of $\procn{Batched Check}$ to verify opened value $\mD$.
        \item If the previous step does not abort, output $(\as{\mU}{i}, \as{\mac{\mU}}{i})$.
    \end{enumerate}
  
  \end{flushleft}
  \end{framed}
\caption{Procedure of Truncation.}
\label{fig:macTruncation}
\end{figure}

 
\paragraph{Non-linear Functions:}
Besides linear functions, ML workloads also include many non-linear functions like ReLU, Softmax, and MaxPooling. In our work, the procedures for those operations are identical to those in the~\cite{spdk2kml}. Please refer to their paper for non-linear functions.


\subsection{Sampling Public Constants}
Our IT MAC compression technique requires functionality that randomly samples public constants from a ring. We implement this functionality by using the summation of previously committed random values as a seed to sample from the ring.

\begin{figure}[htbp!]
    \begin{framed}
    \centerline{\textbf{Functionality} $\funcn{Rand}$}
    \smallskip
    \begin{flushleft}
    %Procedure for truncating the last $p$ bits of an given secret share $\as{x}{}$.\\
    After receiving (\textbf{Rand}) from all parties, sample $r \leftarrow \CipherRing$ and output $r$ to all parties.
  \end{flushleft}
  \end{framed}
\caption{Functionality of Sampling Public Constants.}
\label{fig:randfunc}
\end{figure}


==> archives/3.compacttag.tex <==
\section{\name{}}
\label{sec:compacttag}

In this section, we will describe our matrix multiplication protocol using \name{}. First, we will discuss the compression algorithm. Then, we will describe the tentative IT MAC generation algorithm. With compression algorithm and tentative IT MAC generation, we will discuss the detailed matrix multiplication protocol with \name{}.

\label{sec:mainbody}
\subsection{Tag Compression Procedure}
We use procedure $\procn{Compress}$ to compress large operands into a compact form, reducing the computational complexity for IT MAC computations. Procedure $\procn{Compress}$ takes a 2D matrix as input and will compress the given 2D matrix along the last dimension. The given matrix can be a public constant matrix or a local share of a matrix. Besides the input matrix, $\procn{Compress}$ requires another input matrix $\chi$. $\chi$ is a public constant matrix known to all MPC parties. MPC parties obtain the public constant matrix $\chi$ by invoking $\funcn{Rand}$ beforehand. MPC parties will then use those public random constants to compress the given matrix using linear combinations along the last dimension. Figure~\ref{fig:proccomp} describes the detailed procedure. Note that the public matrix $\chi$ cannot be pre-determined during the offline phase.

\begin{figure}[!htbp]
    \begin{framed}
    \centerline{\textbf{Procedure} $\procn{Compress}$}
    \smallskip

    \begin{flushleft}
    Procedure for compressing a given matrix along its last dimension.\\
    \textbf{\textsc{Inputs:}} 
    
    \begin{itemize}
        \item a matrix $\mM \in \CipherRing^{\sizem \cross \sizen}$ from an MPC party $\party{i}$.
        \item a  public constant matrix $\chi \in \CipherRing^{\sizen\cross 1}$
    \end{itemize}
          
    
    \textbf{\textsc{Compress: }} \\
    \begin{enumerate}
        % \item Each MPC party invokes $\funcn{Rand}$ to obtain $N$ public random constants: $\chi \in \Ring^{N\cross 1} \leftarrow \funcn{Rand}$.
        \item MPC party $\party{i}$ computes $\mU = \mM \mmul \chi$.
    \end{enumerate}

    \textbf{\textsc{Output: }} \\
    \begin{enumerate}
        \item Output $\mU$ to MPC party $\party{i}$.
    \end{enumerate}
   
  \end{flushleft}
%  \vspace{-5mm}
  \end{framed}
\caption{Procedure of Matrix Compression.}
\label{fig:proccomp}
\end{figure}

If a given matrix size is $[\sizem \cross \sizen]$, the compressed matrix size will be $[\sizem\cross 1]$. $\procn{Compress}$ reduces the matrix dimension size by a factor of $\sizen$, and we will see in later sections that reduced operand size will significantly reduce the IT MAC computation complexity by a factor of $\sizen$ as well.


\subsection{Tentative Tag Generation Procedure}
\label{sec:expand}
Another procedure \name{} relies on is $\procn{Expand}$. Given a secretly shared matrix $\as{\mM}{}$, procedure $\procn{Expand}$ will return a secretly shared tentative IT MAC for the given matrix $\as{\mM}{}$. This procedure requires a random authenticated shared matrix $\mR$, and $\procn{Expand}$ will use $\mR$ to generate a regular IT MAC for $\as{\mM}{}$. The detailed procedure is described in Figure~\ref{fig:expand}. To generate a tentative IT MAC for any secret shared matrix $\mM$, MPC parties will first open $\mD=\mR - \mM$. Then, MPC parties compute $\as{\mac{\mM}}{}$ using $\mD$ and the IT MAC of $\mR$. Please note that $\procn{Expand}$ alone is not secure against active adversaries because active adversaries can introduce errors to $\mD$, and procedure $\procn{Expand}$ does not check $\mD$ using any IT MACs. Since $\procn{Expand}$ is not actively secure, our matrix multiplication protocols using $\procn{Expand}$ will use some checking mechanism to verify the correctness of the opened value $\mD$ in order to check the validity of $\as{\mac{\mM}}{}$. In the next section, we will see how matrix multiplication w/ \name{} achieves this goal.

Although procedure $\procn{Expand}$ can indeed generate a tentative IT MAC, $\procn{Expand}$ requires additional broadcasting of $\mD$ and additional authenticated matrix $\mR$ during the offline phase. Luckily, we have made the observation that operations in $\procn{Expand}$ are very similar to operations in $\procn{Truncation}$ (Section~\ref{sec:truncation}). Both procedures take a secret shared input $\as{\mM}{}$, and another random authenticated matrix $(\as{\mR}{}, \as{\mac{\mR}}{})$ ($\hat{\mR}$ for $\procn{Truncation}$) as inputs. Both procedures will output a secretly shared IT MAC by computing $\as{\mac{\mU}}{} = \as{\mac{\mR}}{} - \asmac{i} \cdot \mW$, where $\mW = \mD$ for $\procn{Expand}$, and  $\mW = \frac{\mD}{2^p}$ for $\procn{Truncation}$. Moreover, for ML workloads whose operands are implemented using Fixed Point representations, multiplications are always followed by an $\procn{Truncation}$. Thus, we could merge procedure $\procn{Expand}$ in our \name{} matrix multiplication with its following procedure $\procn{Truncation}$ such that we can avoid the overhead brought by $\procn{Expand}$. Thus, instead of using the $\procn{Expand}$, \name{} matrix multiplication protocol will use $\procn{ExpandTrunc}$ in the Step~\ref{step:multrunc3}. 

\textbf{$\procn{ExpandTrunc}$:}
$\procn{ExpandTrunc}$ takes a secretly shared $\as{\mM}{}$, and two authenticated secret share $(\as{\mR}{i}$, $\as{\mac{\mR}}{i})$ and $(\as{\hat{\mR}}{i}$, $\as{\mac{\hat{\mR}}}{i})$ as inputs, where $\hat{\mR} = \frac{\mR}{2^p}$. $\mR$ and $\hat{\mR}$ are obtained during the offline phase. With the given inputs, $\procn{ExpandTrunc}$ will return the truncated share of $\mM$, and a tentative IT MAC for $\mM$. Steps~\ref{step:exptrunc1} to \ref{step:exptrunc4} in $\procn{ExpandTrunc}$ are similar to those in $\procn{Truncation}$. The correctness of the opened value $\mD$ is not verified in the output stage. Consequently, similar to $\procn{Expand}$, $\procn{ExpandTrunc}$ is only passively secure, and it is the obligation of our matrix multiplication protocol to check the validity of opened value $\mD$. Combining the traits from both $\procn{truncation}$ and $\procn{Expand}$, $\procn{ExpandTrunc}$ is truly a hybrid between them. The detailed procedure is described in Figure~\ref{fig:expandtrunc}.

\begin{figure}[!t]
    \begin{framed}
    \centerline{\textbf{Procedure} $\procn{Expand}$}
    \smallskip

    \begin{flushleft}
    Procedure for generating an expanded IT MAC of a given secret shared matrix $\as{\mM}{}$.\\
    \textbf{\textsc{Inputs:}} 
    
    \begin{itemize}
        \item Secret share $\as{\mM}{i} \in \CipherRing^{\sizem \cross \sizen}$.
        \item An authenticated secret share $(\as{\mR}{i}, \as{\mac{\mR}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$.
    \end{itemize}
    $(\as{\mR}{i}, \as{\mac{\mR}}{i})$ are obtained during the offline phase.
              
    \textbf{\textsc{Expand: }} \\
    \begin{enumerate}
        \item $\party{i}$ computes $\as{\mD}{i} = \as{\mR}{i} - \as{\mM}{i}$.
        \item $\party{i}$ broadcast $\as{\mD}{i}$ such that every party obtain $\mD = \sum_{i=1}^{n} \as{\mD}{i}$
        \label{step:expand4}

        \item $\party{i}$ computes $\as{\mac{\mM}}{i} = \as{\mac{\mR}}{i} - \asmac{i} \cdot \mD$.
        
    \end{enumerate}

    \textbf{\textsc{Output: }} \\
    \begin{enumerate}
        \item Output $\as{\mac{\mM}}{i}$ as a secretly shared tentative IT MAC of $\mM$ to $\party{i}$.
        \item Output $\as{\mac{\mR}}{i}$ to $\party{i}$.
        \item Output $\mD$ to each party.
    \end{enumerate}
  \end{flushleft}
%  \vspace{-5mm}
  \end{framed}
\caption{Procedure of Tag Expansion.}
\label{fig:expand}
\end{figure}


\begin{figure}[!t]
    \begin{framed}
    \centerline{\textbf{Procedure} $\procn{ExpandTrunc}$}
    \smallskip

    \begin{flushleft}
    Procedure for truncating secret shared matrix $\mM$ of last $p$ bits and generating a secret share of truncated $\mM$'s IT MAC.\\

    \textbf{\textsc{Inputs:}} $\party{i}$ has a key $\asmac{i} \in \KeyRing$ and authenticated secret shares: \\
    \begin{itemize}
        \item  $(\as{\mM}{i}, \as{\mac{\mM}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$.\smallskip
        \item  $(\as{\mR}{i}, \as{\mac{\mR}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$.\smallskip
        \item  $(\as{\hat{\mR}}{i}$, $\as{\mac{\hat{\mR}}}{i}) \in (\CipherRing^{\sizem \cross \sizen} \cross \MacRing^{\sizem \cross \sizen})$.
    \end{itemize}
    where  $\hat{\mR} = \frac{\mR}{2^p}$. Authenticated shares of $\mR$ and $\hat{\mR}$ are obtained during the offline phase.  \\
    
    \textbf{\textsc{ExpandTrunc: }} \\
    \begin{enumerate}

        % \item Each $\party{i}$ samples a random matrix $\as{\mQ}{i} \leftarrow \KeyRing^{\sizem \cross \sizen}$.
        % \item Each $\party{i}$ uses authentication procedure in~\cite{spdz2k} to obtain secretly shared tag $\as{\mac{\mQ}}{i}$.
    
        \item $\party{i}$ computes $\as{\mD}{i} = \as{\mR}{i} - \as{\mM}{i}$.
        \label{step:exptrunc1}
        \item $\party{i}$ broadcast $\as{\mD}{i}$ such that every party obtains $\mD = \sum_{i=1}^{n} \as{\mD}{i}$
        \label{step:exptrunc2}
        \item $\party{i}$ computes $\as{\mM}{i} = \as{\hat{\mR}}{i} - \frac{\mD}{2^p}$.
        \label{step:exptrunc3}
        \item $\party{i}$ computes $\as{\mac{\mM}}{i} = \as{\mac{\hat{\mR}}}{i} - \asmac{i} \cdot \frac{\mD}{2^p} $.
        \label{step:exptrunc4}
    \end{enumerate}

    \textbf{\textsc{Output: }} \\
    \begin{enumerate}
        \item Output $(\as{\mM}{i}, \as{\mac{\mM}}{i})$ to $\party{i}$.
        \item Output $\as{\mac{\mR}}{i}$ to $\party{i}$.
        \item Output $\mD$ to each party.
    \end{enumerate}

  \end{flushleft}
%  \vspace{-5mm}
  \end{framed}
\caption{Procedure of Expand Truncation.}
\label{fig:expandtrunc}
\end{figure}




\subsection{Matrix Multiplication with \name{}}
In this section, we will describe our matrix multiplication protocol with \name{}. As described in the previous section, to compute $\mZ = \mX \mmul \mY$, where $\mZ \in  \TextRing^{\sizem \cross \sizeo}$, $\mX\in  \TextRing^{\sizem \cross \sizen}$, and $\mY\in  \TextRing^{\sizen \cross \sizeo}$, each MPC party $\party{i}$ will need to compute the local shares of $\mZ$ and local shares of $\mZ$'s IT MAC using Equation~\ref{eq:compute-z} and Equation~\ref{eq:compute-ztag} respectively.
\begin{align}
    \label{eq:compute-z}
    \as{\mZ}{i} &= \as{\mC}{i} + \mE \mmul \as{\mB}{i} + \as{\mA}{i} \mmul \mU \\
    \label{eq:compute-ztag}
    \as{\mac{\mZ}}{i} &= \as{\mac{\mC}}{i} + \mE \mmul \as{\mac{\mB}}{i} + \as{\mac{\mA}}{i} \mmul \mU
\end{align}
The usage of IT MAC significantly increases the computation cost. Thus, we introduce \name{} to reduce the computation complexity of IT MAC computation. Figure~\ref{fig:matmultrunc} describes procedure $\procn{MatMul}$ with \name{} in details. From Step~\ref{step:multrunc1} to Step~\ref{step:multrunc2} in procedure $\procn{MatMul}$, MPC parties computes local shares of the final matrix product $\as{\mZ}{}$, similar to the state-of-art matrix multiplication (Section~\ref{sec:mlmpc}). Then, MPC parties in Step~\ref{step:multrunc3} invoke $\procn{ExpandTrunc}$ to obtain a truncated matrix product $\as{\hat{\mZ}}{}$ and its corresponding tentative IT MAC $\as{\mac{\hat{\mZ}}}{}$. In Step~\ref{step:multrunc5} and Step~\ref{step:multrunc6}, MPC parties compress necessary operands using the same public constants. Then, from Step~\ref{step:multrunc7} to Step~\ref{step:multrunc8}, MPC parties use compressed operands to compute a \name{} for $\as{\mD}{}$. Those computed compressed IT MACs will then be used to verify the correctness of the tentative IT MACs $\as{\mac{\hat{\mZ}}}{}$ in the output stage.

In the output stage, besides verifying the correctness of $\mE$ and $\mU$, MPC parties will also verify $\mD$ as well. Correctness of $\mE$ and $\mU$ are checked using $\procn{Batched Check}$, and correctness of $\mD$ are checked by broadcasting a special checksum. We later in Section~\ref{sec:security} show that our checksum for $\mD$ has the same probability as $\procn{Batched Check}$ in catching corrupted computation results.

\input{prcedures/compacttag-hybrid}
\input{prcedures/compacttag-hybrid-2}


\textbf{Tag Operation Complexity Analysis:}

\textit{1) Computation Analysis:}
Without \name{}, the resulting IT MAC $\as{\mac{\mZ}}{}$ is computed using Equation~\ref{eq:compute-ztag} whose computational complexity is $\bigOC(\sizem \cross \sizen \cross \sizeo)$. When using \name{}, the resulting IT MAC $\as{\mac{\mZ}}{}$ is no longer computed but generated using a computational lightweight $\procn{ExpandTrunc}$. The computational complexity of $\procn{ExpandTrunc}$ is $\bigOC(\sizem\cross \sizeo)$ because the size of matrix $\as{\mZ}{}$  is $[\sizem\cross \sizeo]$. However, because $\procn{ExpandTrunc}$ is only passive secure, MPC parties need to compute $\as{\mac{\mD}'}{}$ from Step~\ref{step:multrunc7} to Step~\ref{step:multrunc8}. Specifically, a compressed version of $\mZ$'s IT MAC, $\as{\mac{\hat{\mZ}}'}{}$, is computed using Equation~\ref{eq:compute-zcomptag}.

\begin{align}
    \label{eq:compute-zcomptag}
    \as{\mac{\mZ}'}{i} = \as{\mac{\mC}'}{i} + \mE \mmul \as{\mac{\mB}'}{i} + \as{\mac{\mA}}{i}\mmul \mU'
\end{align}
In our \name{} matrix multiplication protocol, many operands are compressed using $\funcn{Rand}$ and $\procn{Compress}$. The size of $\as{\mac{\mB}'}{i}$ and $\mU'$ is $[\sizen\cdot 1]$, a factor of $\sizeo$ reduction compared to their uncompressed version. Thus, the complexity of the matrix multiplication in Equation ~\ref{eq:compute-zcomptag} using compressed operands is $\bigOC(\sizem \cross \sizen)$, reduced by a factor of $\sizeo$ as well. Moreover, the computation complexity of $\procn{Compress}$ is $\bigOC(\sizem\cross \sizeo)$ for $\as{\mac{\mC}'}{}$ and $\bigOC(\sizen\cross \sizeo)$ for $\as{\mac{\mB}'}{}$ and $\mU$. Consequently, combining all the computation complexity from Step~\ref{step:multrunc3} to Step~\ref{step:multrunc8}, the computation complexity of the tag-related operation is $\bigOC(\sizem\cross \sizen + \sizem\cross \sizeo + \sizen\cross\sizeo)$.

\textit{2) Communication Analysis:} 
When using SPD$\nZ_{2^k}$ protocols, MPC parties only need to evaluate Equation~\ref{eq:compute-ztag}, and no tag-related communication is induced. However, when using \name{}, $\procn{Expand}$ induce a round of communication of $[\sizem\cross \sizeo]$ elements. Luckily, we made the observation that we can merge $\procn{Expand}$ and $\procn{Truncation}$. Both procedure $\procn{Expand}$ and $\procn{Truncation}$ induce a round of communication of $[\sizem\cross \sizeo]$ elements. By merging both procedures, the resulting procedure $\procn{ExpandTrunc}$ allows the functionality of tentative IT MAC generation and truncation to share a single round of communication of $[\sizem\cross \sizeo]$ elements, consequently removing added communication of tentative IT MAC generation. Thus, the number of bytes communicated between MPC parties when executing the state-of-art matrix multiplication and truncation protocols are the same as executing $\procn{MatMul}$ with \name{}. 

% Moreover, $\procn{Expand}$ requires MPC parties to prepare additional authenticated shared matrix $\mR$ during the offline phase. Those added communication and extra offline phase workloads are not desirable. However, in the next section, we will show how these overheads can be avoided by merging $\procn{MatMul}$ and $\procn{Truncation}$.

% For SPD$\nZ_{2^k}$ protocols, one only needs to execute $\procn{MatMul}$ in Figure~\ref{fig:mpcmatmul} to perform matrix multiplication. When executing $\procn{MatMul}$ in Figure~\ref{fig:mpcmatmul}, MPC parties need to open $\mE$ and $\mU$ which creates one round of communication of 



% \textbf{$\procn{MatmulTrunc}$:}
% In this section, we will describe the new procedure $\procn{MatmulTrunc}$. $\procn{MatmulTrunc}$ is a procedure that perform operations in both $\procn{Matmul}$ and $\procn{Truncation}$. When using Fixed Point representation to encode operands (precision $p$ bits), MPC parties need to truncate the last $p$ bits of the multiplication product. MPC parties, using $\procn{MatmulTrunc}$, achieve truncation functionality by invoking $\procn{ExpandTrunc}$ to truncate $\as{\mZ}{}$ and generate an expanded IT MAC for $\as{\mZ}{}$. After that, MPC parties compute a compressed IT MAC of $\mD'$ to verify the correctness of opened value $\mD$ so that MPC parties can make sure that the IT MAC $\as{\mac{\mZ}}{}$ is, in fact, computed using correct operands. Details are shown in Figure~\ref{fig:matmultrunc}.



% \textbf{Tag Operation Complexity Analysis for $\procn{MatMulTrunc}$:}

% \textit{1) Computation Analysis:}
% The tag-related computation in $\procn{MatMulTrunc}$ has the same complexity as \name{} $\procn{MatMul}$, which is $\bigOC(\sizem\cross \sizen + \sizem\cross \sizeo)$. They have the same computation complexity because the only difference between them is that one uses $\procn{Expand}$ in Step 3, and the other uses $\procn{ExpandTrunc}$ in Step 3. Moreover, $\procn{ExpandTrunc}$ and $\procn{Expand}$ share the same computation complexity. Consequently, the computational complexity of executing $\procn{MatMulTrunc}$ is $\bigOC(\sizem\cross \sizen + \sizem\cross \sizeo)$, which is significantly less than that of executing SPD$\nZ^{2^k}$ $\procn{MatMul}$ and $\procn{Truncation}$ consecutively.


% \textit{2) Communication Analysis:} 
% $\procn{MatMulTrunc}$ introduce a round of communication of $\sizem\cross \sizeo$ elements in $\procn{ExpandTrunc}$. Thus, the communication cost of executing $\procn{MatMulTrunc}$ is the same as executing SPD$\nZ_{2^k}$ $\procn{MatMul}$ and $\procn{Truncation}$ consecutively.

% In general, Matrix Multiplication with \name{} \textbf{\textit{reduces tag-related computational complexity and incurs no additional overheads in communication and the offline phase}}.

\subsection{Offline Phase Analysis}
\label{sec:offlineanal}
When using the SPD$\nZ_{2^k}$ protocols, one needs to execute $\procn{MatMul}$ and $\procn{Truncation}$ to perform matrix multiplication and truncate the last $p$ bits of the product. When performing $\procn{MatMul}$ and $\procn{Truncation}$, MPC parties needs to execute $\procn{Batched Check}$ three times (twice for $\procn{MatMul}$, and once for $\procn{Truncation}$). Aggregated across all procedures, the following operands are required during the offline phase.
\begin{enumerate}
    \item beaver matrix triple $\mA$, $\mB$ and $\mC$: $\mC = \mA \mmul \mC$.
    \item one pair of authenticated shared matrices $\mR$ and $\hat{\mR}$: $\hat{\mR} = \frac{\mR}{2^p}$.
\end{enumerate}
On the other hand, when using \name{}, one only needs to execute \name{}'s $\procn{MatMul}$ to perform both matrix multiplications and truncation at the same time. $\procn{MatMul}$ executes $\procn{Batched Check}$ twice and $\procn{ExpandTrunc}$ once. Aggregated across all procedures, the following operands are required during the offline phase.
\begin{enumerate}
    \item beaver matrix triple $\mA$, $\mB$ and $\mC$: $\mC = \mA \mmul \mC$.
    \item one pair of authenticated shared matrices $\mR$ and $\hat{\mR}$: $\hat{\mR} = \frac{\mR}{2^p}$.
\end{enumerate}
Comparing SPD$\nZ_{2^k}$ and \name{}, it is obvious that their required materials during the offline phase are identical. Thus, \name{} introduces no overheads for the offline phase.
\subsection{\name{} Convolution}
To convert procedures in Figure~\ref{fig:matmultrunc} to an \name{} Convolution procedure, one needs to replace every matrix multiplication in $\procn{MatMul}$, $\procn{ExtendTrunc}$ and $\procn{Compress}$ with a corresponding Convolution operation. We provide a detailed description of convolution with \name{} in Appendix~\ref{app:conv}.


==> archives/5.evaluations.tex <==
\input{tables/inference}
\input{tables/training}



\section{Experimental Evaluation}
\label{sec:eval}

In this section, we report our experiments and demonstrate our claims empirically.

\subsection{Experimental Setup}
We have evaluated our design on servers with an Intel Xeon Gold 5220R CPU and an Nvidia Quadro RTX 5000. We gather runtime from the average of \textbf{30} iterations of inference or training.

\paragraph{Models Evaluated:} We use ResNet50~\cite{resnet}, a Transformer encoder, and VGG16~\cite{vgg} to evaluate the performance of \name{} against $\SPDZtwok$. VGG16 and ResNet are popular vision models, and Transformer encoders are commonly used in Natural Language Processing models~\cite{bert, roberta, xlm, xlmr}. Those models commonly consist of multiple Transformer encoders of the same configurations. The Transformer configuration we used is the same as BERT~\cite{bert} and XLM~\cite{xlm},  which is $(H=1024, A=16)$.

\paragraph{MPC Setup:} We evaluated  \name{} using 2 sets of MPC parameters: 1) $(k=32, \sigma=26)$ and 2) $(k=64, \sigma=57)$. When using $(k=32, \sigma=26)$, the message space for a matrix $\mM$ will be $\nZ_{2^{32}}^{\sizem \cross \sizen}$. We also choose $s=32$ in such a case. Thus, $\sigma$, the statistical security parameter, is $26 = 32 - log(32+1)$, according to Theorem~\ref{theo:main}. Consequently, with $(k=32, \sigma=26)$, $(\as{\mM}{}, \as{\mac{\mM}}{}, \asmac{}) \in (\nZ_{2^{64}}^{\sizem \cross \sizen} \cross \nZ_{2^{64}}^{\sizem \cross \sizen} \cross \nZ_{2^{32}})$. Similarly, when using $(k=64, \sigma=57)$, $(\as{\mM}{}, \as{\mac{\mM}}{}, \asmac{}) \in (\nZ_{2^{128}}^{\sizem \cross \sizen} \cross \nZ_{2^{128}}^{\sizem \cross \sizen} \cross \nZ_{2^{64}})$. 

\subsection{Implementation}
We implement the online phase of SPD$\nZ_{2^k}$ and \name{} for DNNs on the basis of CrypTen~\cite{crypten2020}, a PyTorch-based~\cite{pytorch} MPC framework. CrypTen provides an easy-to-use API to build DNN models and supports fixed-point operations using the CUDA kernels. However, CrypTen was originally designed for a semi-honest majority MPC protocol and did not separate the online phase and the offline phase. We separated the offline phase and online phase and modified the CrypTen framework such that the MPC operations comply with those specified in~\cite{spdz2k, spdk2kml}. We used the distributed communication backend from PyTorch to establish communication channels between GPUs.

\paragraph{CUDA Matrix Operation Implementation:}  For CUDA matrix multiplication and Convolutions, we follow the same block multiplication technique as CrypTen~\cite{crypten2020} and CrypGPU~\cite{fis} such that 64-bit or 128-bit integer multiplications are carried out using multiple floating point operations. For example, when using double-precision floating points ($52$ bits for the fraction) to carry out computations,  we divide a 64-bit operand into four 16-bit sub-operands. Thus, $32$ bits are required to store the resulting multiplications. Given all operations for matrix multiplication and Convolutions are multiply and accumulate operations when using double-precision floating points, 20 bits ($52-32$)  are left for accumulation, allowing $1048576=2^{20}$ accumulations, which are far more than enough for ML workloads.


\subsection{Online Phase}
\fixme{1)CPU numbers, 2)For GPU Add tables for online comm and runtime, remove theoretical max and red bar from Fig. 10.  3)add table for theoretical max, SPDZ2k and our protocol. 4)Add momentary cost analysis graph for SPDZ2k and us - 5 cents/GB comm + runtime, 5)Add a bar graph for analysing each step, if possible do this for SPDZ2k and theoretical max one. Helps to visually analyse the cost  of each step in the protocols. 6) Mention the setup details, like the processor GPU, memory, etc}

\paragraph{Labelling:} We shows \name{}'s performance improvements for inference and training in Figure~\ref{fig:main-speedups}. Data labeled with \SPDZtwok{} represents our baseline using protocols from~\cite{spdz2k, spdk2kml}. Data labeled with ``{{\name{}$_\textsf{SA}$}}" show the speedup of \name{} when using $\procn{Expand}$ to generate tentative IT MACs. On the other hand, data labeled with ``\name{}'' show the speedup of \name{} when using $\procn{ExpandTrunc}$ to generate tentative IT MACs. 


\input{tables/decomposition-infer}
\input{tables/decomposition-train}

\paragraph{Inference:}
The first row in Figure~\ref{fig:main-speedups} shows the inference performance improvements of \name{} over a 14Gbps network. For the $(k=32, \sigma=26)$ setting, \name{} achieve $1.11$x, $1.22$x, and $1.21$x inference runtime improvement for ResNet, Transformer, and VGG16, respectively. \name{}'s speedup is $92\%$, $96\%$, and $94\%$ of ``TagFree'', the theoretical maximum speedup of \name{}. 

For the $(k=64, \sigma=57)$ setting, all models see a higher performance improvement over the $(k=32, \sigma=26)$ setting. Most noticeably, \name{} achieves $1.31$x speedup for Transformer. When using the $(k=64, \sigma=57)$ setting, the operand bit length doubles $64\rightarrow 128$. For Convolutions and matrix multiplication, computation complexity is quadrupled, whereas the communication cost for opening $\mE$ and $\mU$ are only doubled. Thus, IT MAC-related computation takes a larger portion of the total inference runtime, resulting in \name{}'s higher performance improvements in the $(k=64, \sigma=57)$ setting.

\name{} out performs \name{}$_\textsf{SA}$ in every settings because \name{}$_\textsf{SA}$ introduces additional communication costs. The added communication cost in \name{}$_\textsf{SA}$ creates a performance gap between \name{}$_\textsf{SA}$ and \name{}.


\paragraph{Training:}
The second row in Figure~\ref{fig:main-speedups} shows the training performance improvements of \name{} over a 14Gbps network. For all models and all MPC settings, \name{} has more performance benefits for training than inference. MPC parties only need to perform forward passes on a given model when performing inferences. However, MPC parties must perform both forward and backward passes during training. IT MAC-related computation of matrix multiplication and Convolution makes up less proportion in the forward pass than in the backward pass. For example, non-linear functions such as ReLU and MaxPooling require communication-intensive secret-sharing format conversion (between binary and arithmetic). Such conversions are usually not needed during the backward pass. Thus, the communication costs induced by secret-sharing format conversion make the IT MAC-related computation take a smaller proportion of runtime during the forward pass. Consequently, \name{} will showcase better speedup for training than inference.

Similar to the inference results, \name{} shows better performance improvements in $(k=64, \sigma=57)$, and \name{} out performs \name{}$_\textsf{SA}$ in every settings.




\begin{figure}[!htbp]
  \centering
    \includegraphics[width=7cm]{figures/decomposition.pdf}
  \caption{Transformer's Training Online Phase Runtime Decomposition. \fixme{What do you mean by total communication? Is this the online runtime or the total runtime? If this is only for online phase, then please divide the bar into input sharing, Matrix multiplication over shares, and tag computation over shares during matrix multiplication, and other other operations}}
  \label{fig:decomp}
\end{figure}


\paragraph{Scaling with More Parties \& Faster Networks:}
Speedups showcased in Figure~\ref{fig:main-speedups} are in the 2PC setting. Table~\ref{tab:scale-pc} shows the \name{}'s speedup w.r.t. \SPDZtwok{} with more numbers of participating parties. When scaling to more parties, we assume every party has a point-to-point connection with every other party. The speedups in Table~\ref{tab:scale-pc} are averaged from all three models. 

With more participating parties, communication costs increase linearly while computation costs stay roughly the same. Thus, the proportion of total runtime taken by tag-related computations has decreased. Since \name{} is reducing the tag-related computations, with more parties, the speedup provided by \name{} decreases. Despite deceased speedup, \name{} can still speed up VGG16 training by $1.35$x.






\begin{table}[!htbp]
\centering
\caption{\name{}'s Average Speedup with More Parties.}
\begin{tabular}{|c|c|c|c|c|}
\hline
          & 2PC   & 3PC   & 4PC   & 5PC   \\ \hline
Inference & 1.26x & 1.20x & 1.17x & 1.14x \\ \hline
Training  & 1.38x & 1.32x & 1.28x & 1.25x \\ \hline
\end{tabular}
\label{tab:scale-pc}
\end{table}
On the other hand, \name{} benefits from faster network connections. Figure~\ref{fig:tagVspeed} shows \name{}'s speedups with faster interconnections. The speedup is averaged across 3 models as well. From Figure~\ref{fig:tagVspeed}, we can see that as the interconnection speed increases, the performance improvements of \name{} protocols increase. A faster interconnection speed does not reduce computation runtime but reduces the time spent on data transmission. Reduced communication runtime and constant computation runtime amplify the proportion of IT MAC-related computation in the total runtime. Since \name{}
optimizes IT MAC-related computations, \name{} achieves better performance improvement with faster interconnections. 
% Moreover, the performance differences between \name{}$_\textsf{SA}$ and \name{}$_\textsf{hybrid}$ decreases as the interconnection speed scales. The performance differences of \name{}$_\textsf{SA}$ and \name{}$_\textsf{hybrid}$ is induced by additional broadcasting  in Step~\ref{step:expand4} of Figure~\ref{fig:expand}. Thus, with faster interconnections, this broadcasting will take less time as well, resulting in narrower performance differences between \name{}$_\textsf{SA}$ and \name{}$_\textsf{hybrid}$. We see similar trends for both VGG16 and Transformer when interconnection speed scales. 

\begin{figure}[!htbp]
  \centering
    \includegraphics[width=8cm]{figures/CompactTagVspeed.pdf}
  \caption{\name{}'s Performance Improvements over $\SPDZtwok$ on Different Interconnect Speed.}
  \label{fig:tagVspeed}
\end{figure}


\paragraph{Monetary Impact:}
For $k=64, \sigma=57$, on average ResNet saves 3.17s/image, 9.07s/image. Xformer saves 4.06s/image, 11.78s/image. VGG16 saves 9.49s/image.

\begin{comment}
\input{tables/wan-infer}
\input{tables/wan-train}
\textbf{WAN VS. LAN:}
Table~\ref{tab:waninfer} and~\ref{tab:wantrain} shows the performance improvements of \name{} when using a 14Gbps LAN and a 14Gbps WAN. Table~\ref{tab:waninfer} shows the data for inference, and Table~\ref{tab:wantrain} shows the data for training. The WAN interconnection we are using has a 70ms latency.

Generally, both algorithms of \name{} exhibit reduced performance enhancements when MPC parties are linked via a WAN. In the case of MPC with a LAN connection, the communication cost primarily consists of the data transmission time (calculated as file size divided by bandwidth). However, for MPC connected via a WAN, the communication cost involves both data transmission time and data propagation delay, defined as the time required for a bit to traverse from the source server to the target server. It should be noted that this additional network latency does not alter the computational runtime of the MPC protocols. Due to increased communication cost, the proportion of IT MAC-related computation cost, an area where the \name{} protocol has been significantly optimized, diminishes in the total runtime. Hence, the savings achieved by \name{} are curtailed due to the imposed network latency.


Among all the models, \name{} demonstrates the most significant performance improvements for Transformer when using WAN to interconnect MPC parties. \name{}'s performance improvement for Transformer in the LAN setting is already the best among all test models due to the largest proportion of IT MAC-related computation taken in the total model runtime. Thus, although communication latency is added to the system, IT MAC-related computation still takes a large proportion of MPC Transformer runtime, resulting in the best \name{}'s performance improvement.

Added communication latency also enlarges the performance differences between \name{}$_{\textsf{SA}}$ and \name{}$_{\textsf{hybrid}}$. Unlike our most optimal protocol \name{}$_{\textsf{hybrid}}$, \name{}$_{\textsf{SA}}$ introduces an additional round of communication during the online phase when MPC parties are obtaining tentative IT MACs. This additional communication cost creates a performance difference between \name{}$_{\textsf{SA}}$ and \name{}$_{\textsf{hybrid}}$, and the difference is amplified when MPC parties are interconnected with WAN. For certain system configurations, \name{}$_{\textsf{SA}}$ even shows negative performance improvement compared with the baseline because the saving derived from reduced IT MAC computation is not enough to offset the additional communication overheads. Luckily, our most optimal protocol \name{}$_{\textsf{hybrid}}$ can remove such overhead and always provide a performance improvement over our baseline.
\end{comment}

\paragraph{Power Usage:}
Tables \ref{tab:powinfer} and \ref{tab:powtrain} show the reduction in power usage by \name{} in comparison to SPD$\nZ{2^k}$. It's noteworthy that power usage with different interconnections is very similar, and the power usage of \name{}$_{\textsf{SA}}$ is similar to that of \name{}. Hence, for brevity, only the power usage reduction for \name{} is presented in Tables \ref{tab:powinfer} and \ref{tab:powtrain}. The metric 'power usage' represents the GPU's power consumption during the training and inference phases, with data collected via the Python package, PyJoules~\cite{pyjoules}.


\input{tables/power-infer}
\input{tables/power-train}

Generally, \name{} achieves $21\%$ to $36\%$ power usage reduction. This power usage reduction is primarily due to the decreased computational complexity associated with IT MAC-related calculations. For the SPD$\nZ_{2^k}$ protocols, large uncompressed IT MACs are used to compute sizeable IT MACs. However, when using \name{}, smaller compressed IT MACs are used to compute small IT MACs. Consequently, a significant reduction in power usage is realized due to this decrease in computational complexity.




\subsection{Offline Phase}
The offline phase performance of \name{} was not part of our evaluation. The key enhancement brought forth by \name{} is its optimized IT MAC computation during the online phase. Our novel protocol, incorporating tentative tag expansion with truncation, yields considerable reductions in IT MAC-related computations during the online phase without introducing additional offline overheads (See Section~\ref{sec:offlineanal}). No additional overheads for the offline phase ensure that \name{}'s offline phase remains identical to those in the protocols detailed in~\cite {spdz2k, spdk2kml}. Given that offline phase protocols are extensively studied and well-understood, we discerned no need to assess \name{}'s offline phase in our analysis.
% \fixme{Mention the offline numbers. Are we performing function-dependent or function-independent preprocessing?}

% We did not evaluate the performance of \name{}'s offline phase. \name{}'s main contribution is optimized IT MAC computation during the online phase. Our final protocol, which merges matrix tentative tag expansion with truncation, achieves significant IT MAC-related computation reduction during the online phase without introducing additional preparation. Due to zero added overheads to the offline phase, \name{}'s offline phase is exactly the same as that in~\cite {spdz2k, spdk2kml}. Offline phase protocols are already well-studied, and we did not see any need to evaluate \name{}'s offline phase.



==> archives/tables.tex <==
\begin{table*}[h]
\centering
\caption{\name{} inference online phase with 14Gbps LAN.}
\begin{tabular}{|c||cccc||cccc||cccc|}
\hline
\multirow{3}{*}{Protocol}   & \multicolumn{4}{c||}{ResNet}  & \multicolumn{4}{c||}{Transformer}  & \multicolumn{4}{c|}{VGG16} \\ \cline{2-13} 
 & \multicolumn{2}{c|}{$k=32, \sigma=26$} & \multicolumn{2}{c||}{$k=64, \sigma=57$} & \multicolumn{2}{c|}{$k=32, \sigma=26$} & \multicolumn{2}{c||}{$k=64, \sigma=57$} & \multicolumn{2}{c|}{$k=32, \sigma=26$} & \multicolumn{2}{c|}{$k=64, \sigma=57$} \\ \cline{2-13} 
 & \multicolumn{1}{c|}{s} & \multicolumn{1}{c|}{Imp.} & \multicolumn{1}{c|}{s} & Imp. & \multicolumn{1}{c|}{s} & \multicolumn{1}{c|}{Imp.} & \multicolumn{1}{c|}{s} & Imp. & \multicolumn{1}{c|}{s} & \multicolumn{1}{c|}{Imp.}  & \multicolumn{1}{c|}{s} & \multicolumn{1}{c|}{Imp.}  \\ \hline
SPD$\nZ_{2^k}$ & \multicolumn{1}{c|}{6.80} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{18.76} & - & \multicolumn{1}{c|}{6.23} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{17.04} & - & \multicolumn{1}{c|}{13.42} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{42.4} & - \\  \hline 
\name{}$_{\textsf{SA}}$ & \multicolumn{1}{c|}{6.24} & \multicolumn{1}{c|}{$8.34\%$}  & \multicolumn{1}{c|}{15.96} & $14.89\%$ & \multicolumn{1}{c|}{5.12} & \multicolumn{1}{c|}{$17.74\%$} & \multicolumn{1}{c|}{13.12} & $22.94\%$ & \multicolumn{1}{c|}{11.18} & \multicolumn{1}{c|}{$16.73\%$}  & \multicolumn{1}{c|}{34.18} & $19.49\%$ \\ \hline 
\name{}$_{\textsf{hybrid}}$ & \multicolumn{1}{c|}{6.11} & \multicolumn{1}{c|}{$10.14\%$} & \multicolumn{1}{c|}{15.59} & $16.89\%$ & \multicolumn{1}{c|}{5.04} & \multicolumn{1}{c|}{$18.96\%$} & \multicolumn{1}{c|}{12.98} & $23.77\%$ & \multicolumn{1}{c|}{11.07} & \multicolumn{1}{c|}{$17.54\%$}  & \multicolumn{1}{c|}{32.91} & $22.37\%$ \\ \hline 
Theoretical Max Imp.& \multicolumn{1}{c|}{5.64} & \multicolumn{1}{c|}{$17.15\%$} & \multicolumn{1}{c|}{14.43} & $23.12\%$ & \multicolumn{1}{c|}{4.91} & \multicolumn{1}{c|}{$21.15\%$} & \multicolumn{1}{c|}{12.70} & $25.44\%$ & \multicolumn{1}{c|}{10.37} & \multicolumn{1}{c|}{$22.22\%$}  & \multicolumn{1}{c|}{30.52} & $28.02\%$ \\ \hline
\end{tabular}
\label{tab:infer}
\end{table*}

==> notes/old-proof.tex <==
\textbf{Correctness:} In this section, we will discuss the correctness of computed $\as{\mac{\mZ}}{}$. In procedure $\procn{MatMul}$ with \name{},   $\as{\mac{\mZ}}{}$ is computed by invoking $\procn{Expand}$. In the Step 3 of $\procn{Expand}$, $\as{\mac{\mZ}}{}$ is computed using revealed matrix $\mD$ and local share of $\as{\mac{\mR}}{}$. $\as{\mac{\mR}}{}$ is obtained during the offline phase, and active adversaries cannot introduce errors to the honest parties' $\as{\mac{\mR}}{}$. However, adversaries can introduce errors to the revealed matrix $\mD = \mR - \mZ + \mQ$. Thus, to verify the correctness of $\as{\mac{\mZ}}{}$, MPC parties only need to check the correctness of $\mD$. A compressed IT MAC for $\mD$ is computed in $\procn{MatMul}$. The computed compressed IT MAC of $\mD$ is $\as{\mac{\mD}'}{}$, which equals to $\procn{Compress}\{\as{\mac{\mD}}{}\}$. One can see this using the following equations.
\begin{align}
    \as{\mac{\mD}'}{} &= \as{\mac{\mR}'}{} - \as{\mac{\mZ}'}{} + \as{\mac{\mQ}'}{} \\
     &= \as{\mac{\mR}}{} \mmul \chi - \as{\mac{\mZ}}{} \mmul \chi + \as{\mac{\mQ}}{} \mmul \chi  \\
     &= (\as{\mac{\mR}}{} - \as{\mac{\mZ}}{} + \as{\mac{\mQ}}{}) \mmul \chi \\
     &= \as{\mac{\mD}}{} \mmul \chi
\end{align}
Consequently, the following equations hold for every row of $\mac{\mD}$ and $\mD$:
\begin{align}
   \forall i \in [\sizem]:  \as{\mac{\mD_i}'}{} &= \sum_{j=1}^{\sizeo} \as{\mac{\mD_{i,j}}}{} \cdot \chi_j \\
   \forall i \in [\sizem]:  \as{{\mD'_i}}{} &= \sum_{j=1}^{\sizeo} \as{{\mD_{i,j}}}{} \cdot \chi_j
\end{align}

During the output stage of $\procn{MatMul}$, $\as{\mac{\mD_i}'}{}$ is used to check the during correctness of $\mD$ using $\procn{Batched Check}$ using another random vector $\hat{\chi} \in \CipherRing^{\sizem}$. During this process, each party will compute the following equation:

\begin{align}
    \sum_{i=1}^{\sizem} \sum_{j=1}^{\sizeo}   ( \asmac{} \cdot {\mD_{i,j}}  - \as{\mac{\mD_{i,j}}}{} ) \cdot (\hat{\chi}_i \cdot \chi_j)  
\end{align}
Adversaries can only introduce errors to the broadcasted $\mD_{i,j}$, since $\asmac{}$ and $\as{\mac{\mD_{i,j}}}{}$ is either authenticated local values or derived from authenticated local values. After adding errors, Equation~\ref{eq:localCheck} becomes
\begin{align}
    \label{eq:localCheck}
    \sum_{i=1}^{\sizem} \sum_{j=1}^{\sizeo}   ( \asmac{} \cdot ({\mD_{i,j}}{} + e_{i,j})   - \as{\mac{\mD_{i,j}}}{} ) \cdot (\hat{\chi}_i \cdot \chi_j)  
\end{align}

The opened value by broadcasting Equation~\ref{eq:localCheck} is: 
\begin{align}
    &\sum_{i=1}^{\sizem} \sum_{j=1}^{\sizeo}   ( \mkey{} \cdot (\mD_{i,j} + e_{i,j})   - {\mac{\mD_{i,j}}}) \cdot (\hat{\chi}_i \cdot \chi_j)  \\
    &= \sum_{i=1}^{\sizem} \sum_{j=1}^{\sizeo} ( \mkey{} \cdot \mD_{i,j} + \mkey{} \cdot e_{i,j}   - {\mac{\mD_{i,j}}}) \cdot (\hat{\chi}_i \cdot \chi_j) \\
    &= \sum_{i=1}^{\sizem} \sum_{j=1}^{\sizeo}  \mkey{} \cdot  e_{i,j} \cdot \hat{\chi}_i \cdot \chi_j  \\
    \label{eq:checksum}
    & =\sum_{i=1}^{\sizem} (\hat{\chi}_i \cdot \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j) = 0
\end{align}
MPC parties will check if \ref{eq:checksum} equals $0$. In the next section, we will show the probability of adversaries introducing errors to $\mD$ while \ref{eq:checksum} evaluates $0$. We will use Theorem 1 from~\cite{spdz2k} to support our proof as Lemma 1, re-stated below.

\textbf{Lemma 1.} Suppose that the inputs $\as{x}{1}, ... \as{x}{t}$ to the $\procn{Batched Check}$ procedure are consistent sharings of  ${x}_{1}, ... {x}_{t}$ under the MAC key $\mkey{} = \sum_{i=1}^{n} \asmac{i} \mod \KeyRing$, and the honest parties' shares $\asmac{i} \in \KeyRing$ are uniform random in the view of an adversary corrupting at most $n-1$ parties. Then,
\begin{align}
    & \Pr[ \sum_{i=1}^{t} \chi_{i} \cdot \mac{\mX_i} - \mkey{} \cdot \chi_{i} \cdot (\mX_i + e_i) \modeq{k+s} 0 ] \\
     = &\Pr[ \sum_{i=1}^{t} \mkey{} \cdot \chi_{i} \cdot e_i \modeq{k+s} 0 ] \\
     \leq& 2^{-s + log(s+1)}
\end{align}



With Lemma 1, we will show the probability of adversaries introducing non-zero errors to $\mD$ while \ref{eq:checksum} evaluates to $0$. Let's also write $\sum_{j=1}^{\sizeo}  \mkey{} \cdot e_{i,j} \cdot  \chi_j$ as $g_i$. Thus, probability in Equation~\ref{eq:checksum} can be written as:
\begin{align}
    \label{eq:mainthe}
     &\Pr[ \sum_{i=1}^{\sizem} \hat{\chi}_i \cdot g_i \modeq{k+2s} 0] \\
    =&\Pr[ \sum_{i=1}^{\sizem} \hat{\chi}_i \cdot y_i \modeq{k+2s} 0 \land \forall_{i=1}^{\sizem} g_i \modeq{k+s} y_i] \\
    \leq &min(\Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot y_i \modeq{k+2s} 0], \Pr[\forall_{i=1}^{\sizem}  g_i \modeq{k+s} y_i])
\end{align}
For the first probability, let's assume $2^v$ is the largest power of two dividing $y_i$. We know that $y_i < 2^{k+s}$ by assumption. Thus, we have $v < k+s$. Therefore,

\begin{align}
    &\Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot y_i \modeq{k+2s} 0] \\
   =&\Pr[ \hat{\chi}_{1} \cdot y_{1} \modeq{k+2s} \sum_{i=2}^{\sizem} \hat{\chi}_i \cdot y_i] \\
   =&\Pr[ \hat{\chi}_{1} \cdot \frac{y_{1}}{2^v} \modeq{s} \frac{\sum_{i=2}^{\sizem} \hat{\chi}_i \cdot y_i}{2^v}] \\
   =&\Pr[ \hat{\chi}_{1}   \modeq{s} \frac{\sum_{i=2}^{\sizem} \hat{\chi}_i \cdot y_i}{2^v} \cdot (\frac{y_{1}}{2^v})^{-1}] \\
\leq& 2^{-s}   
\end{align}
For the second probability, we use Lemma 1 to show its probability.

\begin{align}
     \Pr[\forall_{i=1}^{\sizem}  g_i \modeq{k+s} y_i] \leq min_{i=1}^{\sizem} (g_i \modeq{k+s} y_i) \leq 2^{-s + log(s+1)}
\end{align}

Thus, the minimum of those two probabilities is $\Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot y_i \modeq{k+2s} 0]$. Therefore,

\begin{align}
    \label{eq:mainthe}
     &\Pr[ \sum_{i=1}^{\sizem} \hat{\chi}_i \cdot g_i \modeq{k+2s} 0] \leq  \Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot y_i \modeq{k+2s} 0] \leq 2^{-s}
\end{align}

% If the multiplication inside probability~\ref{eq:mainthe} evaluates to $0$, either $\sum_{i=1}^{\sizem} \hat{\chi}_i$ or $\sum_{i=1}^{\sizem} \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j$ should be $0$. Let's denote the event $\forall i \in [\sizem]: \hat{\chi_{i}} = 0 \mod \CipherRing$ as $\event_1$ and denote the event $\forall i \in [\sizem], j \in [\sizeo]: \mkey{} \cdot  e_{i,j} \cdot \chi_{j}  = 0 \mod \CipherRing$ as $\event_2$. Thus, the probability~\ref{eq:mainthe} can be re-written as:
% \begin{align}
%     \Pr[& \sum_{i=1}^{\sizem} \hat{\chi}_i= 0  \mod \CipherRing \lor  \nonumber &&\\ 
%     & \sum_{i=1}^{\sizem} \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j = 0 \mod \CipherRing] &&\\
%     =\Pr[&\event_1 \lor \event_2]&&
% \end{align}
% Since all the elements inside $\hat{\chi}$ are randomly chosen from $\KeyRing$ and $\log_{2}^{\sizem} < k$ is always true, probably of $\event_1$ is $2^{-\sizem \cdot s}$.

% As for $\event_2$,






% \begin{align}
%     & \Pr[ \sum_{i=1}^{\sizem} \hat{\chi}_i \cdot \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j = 0 \mod \CipherRing] \\
%     & = \Pr(\event_E \lor \event_B) \\
%     & = \Pr(\event_E) + \Pr(\event_B) - \Pr(\event_E \land \event_B) \\
%     & = \Pr(\event_E) + \Pr(\event_B) - \Pr(\event_E)j \cdot \Pr(\event_B) \\
%     & \leq \Pr(\event_E) + \Pr(\event_W) - \Pr(\event_E) \cdot \Pr(\event_W) \\
%     & = 2^{-s + log(s+1)} + 2^{-s} -  2^{-s + log(s+1)} \cdot 2^{-s} \\
%     & = (2^{log(s+1)} + 1 - 2^{-s+log(s+1)}) \cdot 2^{-s} \\
%     & \leq  2^{-s +log(2^{log(s+1)} + 1 - 2^{-s+log(s+1)}) }
% \end{align}

% Step 26 holds because $\Pr(\event_B) \leq \Pr(\event_W)$, and step 25 is a monotonous increasing function.
\onecolumn
\subsection{New Proof}


\textit{Lemma} \#1:  Suppose that $\hat{\chi}_1, \hat{\chi}_2, ..., \hat{\chi}_{\sizem}$ are sampled randomly from $\KeyRing$. Adversaries can choose \textbf{\textit{any}} combination of $y_1, y_2, ..., y_{\sizem}$ from $\CipherRing$, where not all $y_i$s are zero modulo $2^{k+s}$. Then, 

\begin{align}
    \Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot y_i \modeq{k+2s} 0] \leq 2^{-s}
\end{align}

\textbf{\textit{Proof:}}
Let's assume $2^v$ is the largest power of two dividing $y_i$. We know that $y_i < 2^{k+s}$ by assumption. Thus, we have $v < k+s$. Therefore,
\begin{align}
    &\Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot y_i \modeq{k+2s} 0] \\
   =&\Pr[ \hat{\chi}_{1} \cdot y_{1} \modeq{k+2s} \sum_{i=2}^{\sizem} \hat{\chi}_i \cdot y_i] \\
   =&\Pr[ \hat{\chi}_{1} \cdot \frac{y_{1}}{2^v} \modeq{s} \frac{\sum_{i=2}^{\sizem} \hat{\chi}_i \cdot y_i}{2^v}] \\
   =&\Pr[ \hat{\chi}_{1}   \modeq{s} \frac{\sum_{i=2}^{\sizem} \hat{\chi}_i \cdot y_i}{2^v} \cdot (\frac{y_{1}}{2^v})^{-1}] \\
\leq& 2^{-s}   
\end{align}

\textit{Lemma} \#2: Suppose that ${\chi}_1, {\chi}_2, ..., {\chi}_{\sizeo}$ are sampled randomly from $\KeyRing$, and $\mkey{}$ are uniformly sampled from $\KeyRing$. Adversaries can choose \textbf{\textit{any}} combination of $e_1, e_2, ..., e_{\sizeo}$ from $\TextRing$, where not all $e_i$s are zero modulo $2^{k}$. Then, 

\begin{align}
    \Pr[\sum_{i=1}^{\sizeo} \mkey{} \cdot e_{i} \cdot  \chi_i \modeq{k+s} 0] \leq 2^{-s+log(s+1)}
\end{align}
Lemma \#2 are proven in~\cite{spdz2k}.

\textbf{Theorem} \#1: Suppose that $\chi_1, \chi_2, ..., \chi_{\sizem}$ and $\hat{\chi}_1, \hat{\chi}_2, ..., \hat{\chi}_{\sizeo}$ are sampled randomly from $\KeyRing$. Adversaries can choose \textbf{\textit{any}} combination of $e_{i,j}$ where not all $e_{i,j}$ are zero modulo $2^k$, and $\sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j$ is in modulo of $2^{k+s}$, such that

\begin{align}
    \Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+2s} 0] \leq 2^{-s+log(s+1)}
\end{align}

\textbf{\textit{Proof:}}
\begin{align}
     &\Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+2s} 0] \\
    =&\Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+2s} 0 | \forall_{i=1}^{\sizem}: \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+s} y_i] \cdot \Pr[\forall_{i=1}^{\sizem}: \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+s} y_i] \\
    \label{eq:conditions}
    =&\Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot y_i \modeq{k+2s} 0]\cdot \Pr[\forall_{i=1}^{\sizem}: \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+s} y_i]
\end{align}
Here, adversaries can choose from two attack schemes: 1) choose $e_{i,j}$ such that \textbf{not all} $y_i$s are zero modulo $2^{k+s}$, and 2) choose $e_{i,j}$s such that \textbf{all} $y_i$s are zero modulo $2^{k+s}$.
In the first case, we will apply lemma \#1 and lemma\#2. Therefore,
\begin{align}
    &\Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot y_i \modeq{k+2s} 0]\cdot \Pr[\forall_{i=1}^{\sizem}: \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+s} y_i]\\
    \leq& 2^{-s} \cdot \Pr[\forall_{i=1}^{\sizem}: \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+s} y_i] \\
    \leq& 2^{-s} \cdot \Pr[\exists_{i=1}^{\sizem}: \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+s} y_i] \\
    \leq& 2^{-s} \cdot  2^{-s+log(s+1)} \\
    \leq& 2^{-s}
\end{align}
In the second case, where adversaries make all $y_i$ zeros, the probability of $\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot y_i \modeq{k+2s} 0$ will equal one. Therefore,
\begin{align}
    &\Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot 0 \modeq{k+2s} 0]\cdot \Pr[\forall_{i=1}^{\sizem}: \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+s} 0]\\
   =&1\cdot \Pr[\forall_{i=1}^{\sizem}: \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+s} 0]\\
   =&\Pr[\forall_{i=1}^{\sizem}: \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+s} 0]\\
   \leq& \Pr[\exists_{i=1}^{\sizem}: \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+s} 0] \\
   \leq&  2^{-s+log(s+1)}
\end{align}
Adversaries will have a better probability in the second case. Thus,
\begin{align}
    \Pr[\sum_{i=1}^{\sizem} \hat{\chi}_i \cdot \sum_{j=1}^{\sizeo} \mkey{} \cdot e_{i,j} \cdot  \chi_j \modeq{k+2s} 0] \leq 2^{-s+log(s+1)}
\end{align}

==> prcedures/compacttag-hybrid-2.tex <==
\begin{figure}[!htbp]
    \begin{framed}
    \centerline{\textbf{Procedure} $\procn{MatMul}$ w/ \name{} (continuation)}
    \smallskip

    \begin{flushleft}
    \algoHead{Verification:} 
    \begin{myenumerate}
        \item Use the {\em tag check} phase from $\procn{\batchcheck}$ to verify the correctness of the reconstructed $\mE, \mU$.
        \item All parties sample a public random matrix $\hat{\chi} \in \KeyRing^{\sizem\cross1}$ via $\funcn{\Rand}$.
        \item Compute $\as{\CS}{} \modeq{k+s} \asmac{} \cdot {\compact{\lsum{\mD}}}$.
        \item Compute $\as{\CS}{} \modeq{k+2s} \as{\CS}{}\ewmul{\hat{\chi}}  -  {\as{\mac{\compact{\mD}}}{}}\ewmul {\hat{\chi}}$.
        \item Commit and open $\as{\cs}{} \modeq{k+2s} \sum_{i=1}^{\sizem} \as{\CS_{i,1}}{}$.
        \item If reconstructed $\cs \neq 0$ modulo $2^{k+2s}$, then abort.
        \item If the previous steps do not abort, output $\shr{\mZ} =(\as{\trunc{\mZ}}{}, \as{\mac{\trunc{\mZ}}}{}, \asmac{})$.
    \end{myenumerate}
    \end{flushleft}
  \vspace{-5mm}
  \end{framed}
  \vspace{-5mm}
\caption{Procedure of Matrix Multiplication using \name{} (continuation).}
\label{fig:matmultrunc2}
\end{figure}

==> prcedures/compacttag-sa.tex <==
\begin{figure}[]
    \begin{framed}
    \centerline{\textbf{Procedure} $\procn{MatMul}$ w/ \name{}}
    \smallskip

    \begin{flushleft}        
    Procedure for performing $\mZ = \mX \mmul \mY$, where $\mZ\in  \TextRing^{\sizem\cross \sizeo}$, $\mX\in  \TextRing^{\sizem\cross \sizen}$, and $\mY\in  \TextRing^{\sizen\cross \sizeo}$. The matrix $\mX$ and $\mY$ are secretly shared and authenticated.
    
    \textbf{\textsc{Inputs:}} The same inputs as Procedure $\procn{Matmul}$.
    
    %     $\party{i}$ has a key $\asmac{i} \in \KeyRing$ and authenticated shares:\\
    % \begin{itemize}
    %     \item  $(\as{\mX}{i}$, $\as{\mac{\mX}}{i}) \in (\CipherRing^{\sizem\cross \sizen} \cross \MacRing^{\sizem\cross \sizen})$. \smallskip
    %     \item  $(\as{\mY}{i}$, $\as{\mac{\mY}}{i}) \in (\CipherRing^{\sizen\cross \sizeo} \cross \MacRing^{\sizen\cross \sizeo})$.\smallskip
    %     \item  $(\as{\mA}{i}$, $\as{\mac{\mA}}{i}) \in (\CipherRing^{\sizem\cross \sizen} \cross \MacRing^{\sizem\cross \sizen})$.\smallskip
    %     \item  $(\as{\mB}{i}$, $\as{\mac{\mB}}{i}) \in (\CipherRing^{\sizen\cross \sizeo} \cross \MacRing^{\sizen\cross \sizeo})$.\smallskip
    %     \item  $(\as{\mC}{i}$, $\as{\mac{\mC}}{i}) \in (\CipherRing^{\sizem\cross \sizeo} \cross \MacRing^{\sizem\cross \sizeo})$.
    % \end{itemize}

    \textbf{\textsc{Matrix Multiplication:}} \\
    \begin{enumerate}
        % \item Each $\party{i}$ execute open phase of Batched Check to open $\as{x-a}{i}$ and $\as{y-b}{i}$ as $\mE$ and  $\mU$, respectively.
        % \item $\party{i}$ computes locally $\as{z}{i} = \as{c}{i} + \mE \cdot \as{b}{i} + \as{a}{i} \cdot \mU$.

        \item Each $\party{i}$ executes open phase of Batched Check to open $\as{\mX-\mA}{i}$ and $\as{\mY-\mB}{i}$ as $\mE$ and  $\mU$, respectively.
        \item $\party{i}$ computes locally $\as{\mZ}{i} = \as{\mC}{i} + \mE \mmul \as{\mB}{i} + \as{\mA}{i} \mmul \mU$.
        \label{step:mul2}
        \item $\party{i}$ invokes $\procn{Expand}$ on $\as{\mZ}{i}$: $\as{\mac{\mZ}}{i}, \as{\mac{\mR}}{i}, \as{\mac{\mQ}}{i}, \mD \leftarrow \procn{Expand}(\as{\mZ}{i})$.        
        \label{step:mul3}
        \item $\party{i}$ invoke $\funcn{Rand}$ to obtain a public constant matrix $\chi \in \CipherRing^{\sizen\cross 1}$.
        \label{step:mul4}
        \item Using the same public constant matrix $\chi$, $\party{i}$ invoke $\procn{Compress}$ on operand $\as{\mac{\mQ}}{i}$, $\as{\mac{\mR}}{i}$, $\as{\mac{\mY}}{i}$, $\as{\mac{\mB}}{i}$, $\as{\mac{\mC}}{i}$, $\mU$, and $\mD$. The resulting compressed operands are $\as{\mac{\mQ}'}{i}$, $\as{\mac{\mR}'}{i}$, $\as{\mac{\mY}'}{i}$, $\as{\mac{\mB}'}{i}$, $\as{\mac{\mC}'}{i}$, $\mU'$, and $\mD'$, respectively.
        \label{step:mul5}
        \item $\party{i}$ computes locally $\as{\mac{\mZ}'}{i} = \as{\mac{\mC}'}{i} + \mE \mmul \as{\mac{\mB}'}{i} + \as{\mac{\mA}}{i} \mmul \mU'$.
        \label{step:mul6}
        \item $\party{i}$ computes locally $\as{\mac{\mD}'}{i} = \as{\mac{\mR}'}{i} - \as{\mac{\mZ}'}{i} + \as{\mac{\mQ}'}{i}$.
        \label{step:mul7}
        \item $\party{i = 1}$ computes locally $\as{\mZ}{i} = \as{\mZ}{i} + \mE \mmul \mU$ and $\as{\mac{\mZ}}{i} = \as{\mac{\mZ}}{i} + \asmac{i} \cdot (\mE \mmul \mU)$.
    \end{enumerate}

    \textbf{\textsc{Output: }} \\
    \begin{enumerate}
        \item Use the Tag Check Phase from the Batched Check to check the validity of opened values: $\mE, \mU$.
        \item All parties collectively sample a public random matrix $\hat{\chi} \in \CipherRing^{\sizem\cross1}$. 
        \item Each $\party{i}$ computes and open $\asmac{i} \cdot \iprod{\mD'}{\hat{\chi}}  -  \iprod{\as{\mac{\mD'}}{i}}{\hat{\chi}}  \in \nZ_{k+2s}$.
        \item If the opened value is not zero modulo $2^{k+2s}$, then abort.
        \item If the previous step does not abort, output $(\as{\mZ}{}, \as{\mac{\mZ}}{})$ to $\party{i}$.
    \end{enumerate}
    \medskip
  \end{flushleft}
  \vspace{-5mm}
  \end{framed}
\caption{Procedure of Matrix Multiplication using \name{}.}
\label{fig:compacttagmul}
\end{figure}

==> tables/decomposition-train.tex <==
\begin{table}[]
\centering
\caption{Training Runtime (seconds/input) Decomposition for $(k=64, \sigma=57)$.}
\begin{tabular}{|c|l|r|r|r|}
\hline
Model                        & Protocol                     & \multicolumn{1}{c|}{IT MAC} & \multicolumn{1}{c|}{Comm} & \multicolumn{1}{c|}{Total} \\ \hline \hline
\multirow{2}{*}{ResNet}      & \SPDZtwok{} & 11.64                       & 9.15                      & 45.99                      \\ \cline{2-5}
                             & \name{}     & \textbf{2.61}                        &   9.12                    & 36.92                      \\ \hline \hline
\multirow{2}{*}{Transformer} & \SPDZtwok{} & 12.56                       & 6.96                      & 40.74                      \\ \cline{2-5} 
                             & \name{}     & \textbf{0.57}                        & 6.87                      & 28.92                      \\ \hline \hline
\multirow{2}{*}{VGG16}       & \SPDZtwok{} & 44.27                       & 12.22                     & 133.73                     \\ \cline{2-5} 
                             & \name{}     & \textbf{2.52}                        & 11.51                     & 93.80                      \\ \hline
\end{tabular}
\label{tab:decomp-train}
\end{table}

==> tables/training.tex <==
\begin{comment}
\begin{table*}[h]
\centering
\caption{\name{} training online phase with 14Gbps LAN.}
\begin{tabular}{|c||cccc||cccc|}
\hline
\multirow{3}{*}{Protocol}   & \multicolumn{4}{c||}{ResNet}  & \multicolumn{4}{c|}{Transformer}  \\ \cline{2-9} 
 & \multicolumn{2}{c|}{$k=32, \sigma=26$} & \multicolumn{2}{c||}{$k=64, \sigma=57$} & \multicolumn{2}{c|}{$k=32, \sigma=26$} & \multicolumn{2}{c|}{$k=64, \sigma=57$} \\ \cline{2-9} 
 & \multicolumn{1}{c|}{s} & \multicolumn{1}{c|}{Imp.} & \multicolumn{1}{c|}{s} & Imp. & \multicolumn{1}{c|}{s} & \multicolumn{1}{c|}{Imp.} & \multicolumn{1}{c|}{s} & Imp.   \\ \hline
SPD$\nZ_{2^k}$ & \multicolumn{1}{c|}{17.65} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{45.99} & - & \multicolumn{1}{c|}{14.15} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{40.41} & - \\  \hline 
\name{}$_{\textsf{SA}}$ & \multicolumn{1}{c|}{15.2} & \multicolumn{1}{c|}{$13.78\%$}  & \multicolumn{1}{c|}{38.15} & $17.05\%$ & \multicolumn{1}{c|}{10.37} & \multicolumn{1}{c|}{$26.71\%$} & \multicolumn{1}{c|}{29.28} & $27.52\%$ \\ \hline 
\name{}$_{\textsf{hybrid}}$ & \multicolumn{1}{c|}{14.82} & \multicolumn{1}{c|}{$16.04\%$} & \multicolumn{1}{c|}{36.92} & $19.72\%$ & \multicolumn{1}{c|}{10.29} & \multicolumn{1}{c|}{$27.29\%$} & \multicolumn{1}{c|}{28.83} & $28.63\%$  \\ \hline
Theoretical Max Imp. & \multicolumn{1}{c|}{14.32} & \multicolumn{1}{c|}{$18.85\%$} & \multicolumn{1}{c|}{34.39} & $25.22\%$ & \multicolumn{1}{c|}{9.58} & \multicolumn{1}{c|}{$29.83\%$} & \multicolumn{1}{c|}{27.28} & $32.48\%$  \\ \hline
\end{tabular}
\label{tab:train}
\end{table*}
\end{comment}

% \begin{figure*}[htbp]
%   \centering

%   \caption{\name{} Training Speedups.}
%   \label{fig:train-speedups}
% \end{figure*}

==> tables/wan-infer.tex <==
\begin{table}[h]
\centering
\caption{\name{} inference online phase performance improvements with 14Gbps LAN \& WAN.}
\begin{tabular}{|c|cccc|}
\hline
\multirow{3}{*}{Protocol}   & \multicolumn{4}{c|}{ResNet}                                                                       \\ \cline{2-5} 
                            & \multicolumn{2}{c||}{$k=32,\sigma=26$}                     & \multicolumn{2}{c|}{$k=64,\sigma=57$} \\ \cline{2-5} 
                            & \multicolumn{1}{c|}{LAN}    & \multicolumn{1}{c||}{WAN}    & \multicolumn{1}{c|}{LAN}     & WAN    \\ \hline
\name{}$_{\textsf{SA}}$     & \multicolumn{1}{c|}{8.34$\%$}  & \multicolumn{1}{c||}{-1.24$\%$} & \multicolumn{1}{c|}{14.89$\%$}  & 8.31$\%$  \\ \hline
\name{}$_{\textsf{hybrid}}$ & \multicolumn{1}{c|}{10.14$\%$} & \multicolumn{1}{c||}{3.90$\%$}  & \multicolumn{1}{c|}{16.89$\%$}  & 12.07$\%$ \\ \hline\hline
\multirow{3}{*}{Protocol}   & \multicolumn{4}{c|}{Transformer}                                                                  \\ \cline{2-5} 
                            & \multicolumn{2}{c||}{$k=32,\sigma=26$}                     & \multicolumn{2}{c|}{$k=64,\sigma=57$} \\ \cline{2-5} 
                            & \multicolumn{1}{c|}{LAN}    & \multicolumn{1}{c||}{WAN}    & \multicolumn{1}{c|}{LAN}     & WAN    \\ \hline
\name{}$_{\textsf{SA}}$     & \multicolumn{1}{c|}{17.74$\%$} & \multicolumn{1}{c||}{11.73$\%$} & \multicolumn{1}{c|}{22.94$\%$}  & 19.72$\%$ \\ \hline
\name{}$_{\textsf{hybrid}}$ & \multicolumn{1}{c|}{18.96$\%$} & \multicolumn{1}{c||}{12.88$\%$} & \multicolumn{1}{c|}{23.77$\%$}  & 20.55$\%$ \\ \hline\hline
\multirow{3}{*}{Protocol}   & \multicolumn{4}{c|}{VGG16}                                                                        \\ \cline{2-5} 
                            & \multicolumn{2}{c||}{$k=32,\sigma=26$}                     & \multicolumn{2}{c|}{$k=64,\sigma=57$} \\ \cline{2-5} 
                            & \multicolumn{1}{c|}{LAN}    & \multicolumn{1}{c||}{WAN}    & \multicolumn{1}{c|}{LAN}     & WAN    \\ \hline
\name{}$_{\textsf{SA}}$     & \multicolumn{1}{c|}{16.73$\%$} & \multicolumn{1}{c||}{5.95$\%$}  & \multicolumn{1}{c|}{19.49$\%$}  & 15.54$\%$ \\ \hline
\name{}$_{\textsf{hybrid}}$ & \multicolumn{1}{c|}{17.54$\%$} & \multicolumn{1}{c||}{8.63$\%$}  & \multicolumn{1}{c|}{22.37$\%$}  & 17.33$\%$ \\ \hline
\end{tabular}
\label{tab:waninfer}
\end{table}

==> tables/wan-train.tex <==
\begin{table}[h]
\centering
\caption{\name{} training online phase performance improvements with 14Gbps LAN \& WAN.}
\begin{tabular}{|c|cccc|}
\hline
\multirow{3}{*}{Protocol}   & \multicolumn{4}{c|}{ResNet}                                                                       \\ \cline{2-5} 
                            & \multicolumn{2}{c||}{$k=32,\sigma=26$}                     & \multicolumn{2}{c|}{$k=64,\sigma=57$} \\ \cline{2-5} 
                            & \multicolumn{1}{c|}{LAN}    & \multicolumn{1}{c||}{WAN}    & \multicolumn{1}{c|}{LAN}     & WAN    \\ \hline
\name{}$_{\textsf{SA}}$     & \multicolumn{1}{c|}{13.78$\%$} & \multicolumn{1}{c||}{-4.74$\%$} & \multicolumn{1}{c|}{17.05$\%$}  & 5.21$\%$  \\ \hline
\name{}$_{\textsf{hybrid}}$ & \multicolumn{1}{c|}{16.04$\%$} & \multicolumn{1}{c||}{2.97$\%$}  & \multicolumn{1}{c|}{19.72$\%$}  & 14.88$\%$ \\ \hline\hline
\multirow{3}{*}{Protocol}   & \multicolumn{4}{c|}{Transformer}                                                                  \\ \cline{2-5} 
                            & \multicolumn{2}{c||}{$k=32,\sigma=26$}                     & \multicolumn{2}{c|}{$k=64,\sigma=57$} \\ \cline{2-5} 
                            & \multicolumn{1}{c|}{LAN}    & \multicolumn{1}{c||}{WAN}    & \multicolumn{1}{c|}{LAN}     & WAN    \\ \hline
\name{}$_{\textsf{SA}}$     & \multicolumn{1}{c|}{26.71$\%$} & \multicolumn{1}{c||}{10.95$\%$} & \multicolumn{1}{c|}{27.52$\%$}  & 23.55$\%$ \\ \hline
\name{}$_{\textsf{hybrid}}$ & \multicolumn{1}{c|}{27.29$\%$} & \multicolumn{1}{c||}{14.39$\%$} & \multicolumn{1}{c|}{28.63$\%$}  & 24.29$\%$ \\ \hline
\end{tabular}
\label{tab:wantrain}
\end{table}
